Heuristic Adaptability to Input Dynamics for SpMM on GPUs

Sparse Matrix-Matrix Multiplication (SpMM) has served as fundamental components in various domains. Many previous studies exploit GPUs for SpMM acceleration because GPUs provide high bandwidth and parallelism. We point out that a static design does not always improve the performance of SpMM on different input data (e.g., >85\% performance loss with a single algorithm). In this paper, we consider the challenge of input dynamics from a novel auto-tuning perspective, while following issues remain to be solved: (1) Orthogonal design principles considering sparsity. Orthogonal design principles for such a sparse problem should be extracted to form different algorithms, and further used for performance tuning. (2) Nontrivial implementations in the algorithm space. Combining orthogonal design principles to create new algorithms needs to tackle with new challenges like thread race handling. (3) Heuristic adaptability to input dynamics. The heuristic adaptability is required to dynamically optimize code for input dynamics. To tackle these challenges, we first propose a novel three-loop model to extract orthogonal design principles for SpMM on GPUs. The model not only covers previous SpMM designs, but also comes up with new designs absent from previous studies. We propose techniques like conditional reduction to implement algorithms missing in previous studies. We further propose DA-SpMM, a Data-Aware heuristic GPU kernel for SpMM. DA-SpMM adaptively optimizes code considering input dynamics. Extensive experimental results show that, DA-SpMM achieves 1.26x~1.37x speedup compared with the best NVIDIA cuSPARSE algorithm on average, and brings up to 5.59x end-to-end speedup to applications like Graph Neural Networks.

==> DAC 2022 - SpMM (arXiv) (1)/data/background.tex <==


\section{Related Works}\label{sec:relatedwork}

\subsection{Design Principles for Sparse}
TVM~\cite{chen2018tvm} uses affine-loop transformation which describes orthogonal design principles for dense tensor operations. Such a framework cannot handle sparse tensor operations with input-dependent loop boundaries. %In terms of sparse tensor operations, 
TACO~\cite{taco} proposes the sparse iterations space and a set of transformation primitives to support tuning. Unfortunately, TACO fails to consider some key techniques (\textit{e.g.,} parallel reduction and GPU shared memory) in their current framework, losing big room for optimization.

\subsection{SpMM Optimization Techniques}
% Under the existing GPU hardware architecture and data structure, how to accelerate the calculation of SpMMul is a very important issue in current research. The parallel programming model of GPU has its richness and complexity, such as thread arrangement and allocation, shared memory and cache model, warp scheduling and synchronization, etc. Therefore, researchers will start from these dimensions to think about more optimized hardware acceleration algorithms.

Bell \textit{et al.}~\cite{bell2009implementing} proposed a set of GPU SpMV implementations including Scalar-CSR and Vector-CSR, and the latter one can utilize idle GPU thread with a parallel reduction technique. GraphBLAS~\cite{graphblas} and GE-SpMM~\cite{gespmm} extend Scalar-CSR to SpMM scenario. CSR-Stream~\cite{greathouse2014efficient} and MergePath~\cite{merrill2016merge} handles workload balancing by introducing corresponding techniques, which work well for sparse matrices with the skewed row-length distribution. However, none of these works enable parallel reduction for SpMM and even combine parallel reduction with workload balance for skewed matrices on GPUs with high parallelism.

\subsection{Input-Adaptive Kernel Selection}%Data Characteristic Analysis for SpMMul}

% Many previous studies focus on how to select kernel implementations based on input characteristics. Their approaches are either analytical rules or a data-driven learning approach. % revealed the influence of data characteristics on the algorithm. They can be divided into two categories: designing sparse formats to assist efficient memory operations on GPUs, and designing algorithms to adapt to various characteristics. 


% The first is to modify the data and study a new data reorganization method to adapt to the GPU's cache mechanism. Aktemur \textit{et al.}~\cite{aktemur2018sparse} proposes an effective loop unroll method and a variation of CSR as the storage format to speedup SpMV with low preprocessing cost. ASpT~\cite{aspt} achieved the adaptive tiling by preprocessing the CSR format sparse matrices and reordering the non-zero elements in column segments in sparse and dense blocks. Peng Jiang et al. \cite{jiang2020novel} further optimize the sparse tiling by row reordering to place similar rows close to each other thus providing better temporal locality for the values of the dense matrix. 
% In terms of adapting algorithms to sparse characteristics, CSR-Adaptive~\cite{greathouse2014efficient} is a method to choose between CSR-Stream and CSR-Vector in granularity of row panels. GraphBlas~\cite{graphblas} designed two SpMM algorithms, RowSplit and MergeSpMM, and made choices according to a threshold on the average row length observed from experiments. GE-SpMM~\cite{gespmm} decides the thread-coarsening strategy according to the width of the dense matrix. %designed a data-aware scheduler based on the feature size of the dense matrix, which could select different coarse-grained algorithms.
% The second is to build a scheduler from data to different algorithms. For example, in the work of Greathouse \textit{et al.}~\cite{greathouse2014efficient} we mentioned before also introduces a novel method called CSR-Adaptive, which determines whether to use CSR-Stream or traditional vector CSR is based on different row lengths. GraphBLAST~\cite{graphblast} designs and implements the key primitives of sparse linear algebra, such as SpMV and SpMM. In the SpMM primitive, GraphBLAST adaptively uses different tactics like row-split and merge path, due to different mean row lengths in sparse matrices. This algorithm adjustment for different sparse matrix characteristics so as to tackle the load imbalance problem more efficiently. GE-SpMM~\cite{gespmm} performs SpMM-like operation on sparse matrices represented in the most common Compressed Sparse Row (CSR) format. GE-SpMM designs a data-aware scheduler based on the feature size of the dense matrix, which could select different coarse-grained algorithms.
% These studies perform primary design choices according to problem characteristics that can be accessed easily. However, the simple rules can be suboptimal for complex design choices like we present in this paper. 

% \subsection{SpMMul based on Model driven auto-tuning}

%GraphBLAS~\cite{graphblas} makes choices between RowSplit and MergeSpMM according to a threshold on the average row length. GE-SpMM~\cite{gespmm} decides the thread-coarsening strategy according to the width of the dense matrix.
Choi \textit{et al.}~\cite{choi2010model} searches for optimal format and different binning strategies. Such heuristics over-simplify input dynamics to one or a few features. Nisa \textit{et al.}~\cite{Nisa2018} explores various ML models for format selection of sparse tensor kernels. SpTFS~\cite{10.5555/3433701.3433724} explores deep learning to select a sparse tensor format. No prior work has studied machine learning techniques for general SpMM tuning.



==> DAC 2022 - SpMM (arXiv) (1)/data/baseline.tex <==


\section{Motivation}\label{sec:baseline}


This section introduces the definition with a conceptual dataflow for SpMMul. Then, we conduct a comprehensive study on previous SpMMul optimizations with thorough controlled experiments, showing that previous SpMMul techniques do suffer from input dynamics.

\subsection{SpMMul Definition}\label{sec:baseline:definition}

Both SpMV and SpMM can be unified with Equation~(\ref{equ:Y=AX}):

\vspace{-5pt}
\begin{equation}\label{equ:Y=AX}
    A_{M\times K} \cdot X_{K\times N} = Y_{M\times N}
\end{equation}

A sparse matrix $A_{M\times K}$ is multiplied by a dense matrix $X_{K\times N}$ to form a dense output matrix $Y_{M\times N}$. Specifically, we have $N=1$ for SpMV, and $N>1$ for SpMM. Previous studies show that, SpMMul is one of the most used and time-consuming operations in applications such as Graph Neural Networks (GNNs)~\cite{gespmm, lin2021accelerating}. We illustrate the SpMMul problem in Figure~\ref{fig:overall}(a), a typical dataflow of SpMMul is to calculate each element of the output matrix, $Y[m, n]$, by calculating the inner-product between the $m$-th row of $A$ and the $n$-th column of $X$. For each row of $A$, elements are sparsely distributed. Thus, corresponding elements in a column of $X$ are selected.

We summarize the dataflow with a sequential implementation for the SpMMul problem into three loops, as is shown in Figure~\ref{fig:overall}(b). The outermost loop is the $M$-Loop, which traverses rows of matrix $A$, specifying the row index $m$ of the output matrix $Y$, shown in Figure~\ref{fig:overall}(c). The next loop is the $N$-Loop, which traverses columns of $X$, specifying the column index $n$ of $Y$, shown in Figure~\ref{fig:overall}(d). Then, the innermost loop is the $K$-Loop, which traverses non-zero elements {$k_1^{(m)},k_2^{(m)},...,k_{K(m)}^{(m)}$} in $A$ and their corresponding elements in $X$, shown in Figure~\ref{fig:overall}(e). Parallelism exists in three loops. Optimizing SpMMul is then simplified into mapping these loops to parallel workers on GPUs (e.g., warps/threads) efficiently.

%Figure~\ref{fig:overall} illustrates the inner-product version of the dataflow of the SpMMul problem, and we will further use it to illustrate the design space throughout Section~\ref{sec:designspace}. This abstraction is generalized to outer-product dataflow in Section~\ref{sec-designspace-unify}, and we show that our statements of the design space remain valid.

%A naive parallel implementation of SpMMul based on GPUs can be described as followed: each thread computes one output in $Y$, which is the dot product of a sparse row vector of $A$ and a dense column vector of $X$. Threads within a warp are organized by unfolding M-Loop, which means threads in the same warp shares the same sparse row of $A$ and computes warpsize elements in the corresponding row of $Y$. $A$ and $X$ are stored in the global memory. Each non-zero element in $A$ is requested by N times, leadint to $nnz*N$ times of global requests. Each element in $X$ is requested by M times, leading to $M*N*K$ times of global requests, which adds up to a large number of global memroy access.

%\mentioned{Similar to a dataflow graph of a program, our graphic notation uses node to represent values and the operation which produces it, and edges to represent dataflow. Our notation however is distinctive from DFG because we use two types of dataflow, i.e., access indirection and computation. Access indirection, the dashed arrows in Fig.~\ref{fig:overall}, represents that loading the destination node value requires an address computed from the source node, i.e. an indirect load dependent on the source. Computation edges, the other arrows are the same as in the DFG, meaning the data dependency of arithmetic operations. As shown in the figure, SpMMul computation involves access indirection from the meta data of each non-zero element, to the corresponding value in the rhs matrix. The metadata itself can be indirectly accessed from the higher level of the data structure, e.g., pointers of the CSR format. The dataflow is the multiplication between non-zero and RHS values, and the sum reduction in the inner-product, which yields the final results.}


%\subsection{Related Works}\label{sec:baseline:relatedwork}






% \section{Optimization on SpMMul}\label{sec:baseline:opt}

% Previous works have proposed several optimization methods for SpMMul on GPUs, and we do a comprehensive survey on these methods in this section.

\subsection{SpMMul Optimizations}

\subsubsection{Shared Memory.}\label{sec:baseline:opt:sharedmemory}

%\textbf{Motivation:}
The shared memory is software-controlled scratchpad memory private to each thread block. Storing frequently-visited data into the shared memory for reuse can effectively reduce access latency and off-chip traffic.

\textbf{Approach:} In SpMMul, a sparse-matrix element $A[m,k]$ can be reused to multiply with different columns of the dense matrix, \textit{i.e.,} $X[k,n]$ for different $n$. To exploit this inter-thread reuse GE-SpMM~\cite{gespmm}, uses the following approach: First load sparse elements in the same row, $k_1^{(m)},...,k_{K(m)}^{(m)}$, altogether into the shared memory. Next, assign parallel threads to compute $Y[m, n]$ with different $n$ by iterating over the $k^{(m)}$'s in the shared memory, shown in Figure~\ref{fig:optimization}(a).

\textbf{Evaluation setup:} We evaluate this technique with a set of 27 sparse matrices, synthesized by R-MAT generator~\cite{chakrabarti2004r} with different matrix sizes, average row-length, and row-length variance. We use the open-source code of GE-SpMM~\cite{gespmm, codegespmm} and test on three GPUs described in Section~\ref{sec:exp:setup}.

\textbf{Results:} GE-SpMM's shared memory optimization improves performance on all 27 matrices and 3 GPUs, with average \textbf{1.20$\times$}, \textbf{1.32$\times$}, \textbf{1.13$\times$} on RTX 3090, RTX 2080, Tesla V100, respectively.

% In devices like Nvidia GPUs, the memory hierarchy can be simplified as followed: each thread has its private local memory, each thread block has shared memory which can be read and written by all the threads in the block, and all the threads on the device have access to the same global memory.

% Acting as a block-level cache for global memory, shared memory technique can be utilized to reduce the bandwidth consumption and improve the computational efficiency on such bandwidth-bounded scenarios. In SpMMul, each output in $Y$ is computed by the dot product of a sparse row vector of $A$ and a dense column vector of $X$, which is a large number of load requests. We can ensure regular access to the density matrix $X$, which is decided by the way we store the matrix(row-major or column-major), making it suitable for achieving high parallelism and bandwidth utilization. But the sparsity of matrix $A$ leads to irregular access patterns of global memory. By making threads within a warp loading the non-zero elements of $A$ into shared memory, we reduce the number of global memory loading requests by a factor of warp-size, which brings significant speedup on such bandwidth-limited scenario. The benefits of introducing shared memory is illustrated in figure \ref{fig:shm}. The average speedup by shared memory on ? graphs is 

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.48\textwidth]{figure/benefits_shared_memory.pdf}
%    \caption{speedup with shared memory technique on GTX 1080Ti and RTX 2080.}
%    \label{fig:shm}
%\end{figure}

\begin{figure*}[!tp]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/optimization.pdf}
    \vspace{-10pt}
    \caption{Previous SpMMul optimization on GPUs. (a) Shared Memory. (b) Thread Coarsening. (c) Vectorized Loading. (d) Tiling.}
    %\vspace{-10pt}
    \label{fig:optimization}
\end{figure*}


\subsubsection{Thread Coarsening.}\label{sec:baseline:opt:coarsening}

%\textbf{Motivation:}
By converting originally parallel workloads to a single sequential thread, one can re-use the loaded data as operands for more computation. This technique, named thread coarsening, reduces the amount of memory access. Prior work observes the memory bandwidth is saturated by excessive memory access when $N$ is large in SpMMul~\cite{gespmm}, which motivates the application of thread coarsening.

\textbf{Approach:} The thread coarsening optimization exploits the insight that sparse-matrix element $A[m,k]$ can be re-used for $Y[m,n]$ with different $n$, similar to the observation in the shared memory technique. Prior work~\cite{gespmm} makes each thread compute two output elements $Y[m,n]$ and $Y[m, n+D]$ where the stride $D$ is set, shown in Figure~\ref{fig:optimization}(b). 

\textbf{Evaluation setup:} We evaluate this technique with the same set of synthesized sparse matrices as in the previous subsection. We compare no-optimization (each thread computes one output element) with GE-SpMM's default implementation where each thread produces two output elements. 

\textbf{Results:} GE-SpMM's thread coarsening optimization brings speedup on 7, 25, and 10 matrices on three GPUs respectively, out of all 27 matrices. The technique causes \textbf{0.94$\times$, 0.98$\times$} degradation on Tesla V100 and RTX 3090, but gives average \textbf{1.20$\times$} speedup on RTX 2080 because RTX 2080 has relatively low memory bandwidth and is sensitive to traffic reduction optimizations. 
% Thread Coarsening is another technique commonly used on GPUs. Normally we want to exploit the highest parallelism when executing on GPUs, but it may lead to redundant memory access. Through thread coarsening, we can merge multiple threads into one, allowing re-use of data and reduce bandwidth consumption. If the task is bandwidth-bounded rather than computation-bounded, the increased memory efficiency may outweigh reduced parallelism and achieve better performance. 

\begin{table*}[!tp]
    \centering
    \vspace{-10pt}
    \caption{Review of optimizations for SpMMul on GPUs with controlled experiments (Min.-Avg.-Max.)}
    \vspace{-5pt}
      \begin{tabular}{c|c|c|c|c|c|c|c}
      \hline
      \multirow{2}[4]{*}{} & \multicolumn{4}{c|}{Reference}      & \multicolumn{3}{c}{Speedup w/ the optimization technique} \\
  \cline{2-8}          & \cite{hong2018efficient}   & \cite{aspt}, \cite{jiang2020novel}   & \cite{gespmm}   & \cite{sputnik}, \cite{wang2020sparsert}   & RTX 3090 & RTX 2080 & Tesla V100 \\
      \hline
      Shared memory & \checkmark   & \checkmark   & \checkmark   & \checkmark   & \underline{0.96}-1.20-1.68 & 1.09-1.32-2.02 & 1.03-1.13-1.36 \\
      Thread coarsening &       & \checkmark   & \checkmark   & \checkmark   & \underline{0.82}-\underline{0.98}-1.25 & \underline{0.61}-1.20-1.50 & \underline{0.75}-\underline{0.94}-1.20 \\
      Vertorized loading & \checkmark   &       &       & \checkmark   & 1.09-1.55-2.15 & 1.41-1.72-1.93 & \underline{0.92}-1.44-1.77 \\
      Tiling* & \checkmark   & \checkmark   &       &       & \underline{0.54}-\underline{0.86}-1.00 & \underline{0.63}-\underline{0.92}-1.06 & \underline{0.67}-\underline{0.91}-1.01 \\
      \hline
      \multicolumn{8}{l}{\small{*Use synthesized block-sparse matrices. Others use R-MAT matrices.}}\\
      \end{tabular}%
    \label{tab:opt}%
    \vspace{-5pt}
  \end{table*}%

\subsubsection{Vectorized Loading.}
%load连续的情况下，一个float2好于两个float

%\textbf{Motivation:}
Vectorized load instructions refer to loading 8 or 16 bytes per thread in one instruction, in form of \texttt{float2, float4}, etc. In applications with excessive random access, vector loading can increase the amount of effective data per request and improve bandwidth efficiency. 

\textbf{Approach:} Sputnik~\cite{sputnik,codesputnik} proposed careful designs to use vector loading for sparse and dense elements. Regarding sparse elements, if the sparse matrix rows are long enough to fill two \texttt{float}-load instructions, Sputnik uses \texttt{float2}-load combined with alignment techniques to load sparse rows efficiently. Regarding dense elements, vector loading can be applied to consecutive $X$ elements in a row.

\textbf{Evaluation setup:} Exploiting the aforementioned insight that each $A[m,k]$ can be used to multiply $X[k,n]$ for all $n$, we make a thread to loading $X[k,0],X[k,1]$ in form of \texttt{float2} if $X$ has a row-major layout, and compare it with the version using 2 \texttt{float} instructions. We implement this comparison on top of a classic SpMV implementation CSR-vector~\cite{bell2009implementing}, and test on the same matrix set as used in previous two subsections, shown in Figure~\ref{fig:optimization}(c).

\textbf{Results:} Vectorized loading brings \textbf{1.55$\times$}, \textbf{1.72$\times$}, \textbf{1.44$\times$} speedup on 3 GPUs respectively in the experiment described above. The vectorized loading benefits performance except for one case on Tesla V100 (0.92$\times$ degradation).

\subsubsection{Tiling.}
%\textbf{Motivation:}
Tiling can enhance the data re-use in matrix-multiplication and effectively reduce off-chip traffic. Coarse-grained tiling methods group sparse elements into 2-D grid to exploit the locality of the pointed dense tiles. Fine-grained sparse-matrix tiling is based on the insight that each dense element $X[k, n]$ can be re-used to multiply $A[m, k]$ with different $m$, and this re-use chance further reduces traffic for $X$.

\textbf{Approach:} Tiling the sparse matrix is challenging because retrieval of $A[m, k]$ with the same $k$ is difficult under row-wise compressed CSR format. ASpT~\cite{aspt} proposed to detect and mark the sparse-matrix elements belonging to the same column $k$. Through their special format, element $X[k, n]$ can be re-used for multiplying $A[m, k]$ with the same $k$ and different $m$, if the number of such $A[m, k]$ exceeds a threshold. The synchronization after collaboratively loading $X[k,:]$ into shared memory is the overhead of this optimization.

\textbf{Evaluation setup:} The sparse-matrix tiling proposed by ASpT~\cite{aspt} targets the sparsity pattern with vertical non-zero vectors, which rarely exists in random matrices generated by R-MAT. Thereby we evaluate this optimization on a set of 9 synthesized block-sparse matrices, with block size {8,16,32} and matrix size {1k, 4k, 20k}. We modify the source code~\cite{codeaspt} of ASpT to disable the preprocessing for comparison. 

\textbf{Results:} ASpT's approach brings speedup on 3, 5, 2 matrices on 3 GPUs, respectively, out of 9 matrices in the set. The average effect is \textbf{0.86$\times$}, \textbf{0.92$\times$}, \textbf{0.91$\times$} after applying the design, while in some cases the technique brings 1.06$\times$ speedup. %We confirm through this experiment that the sparse tiling technique needs to be applied selectively.
% Matrix tiling is a technique that is often utilized to reduce bandwidth and is of more efficiency when the data exhibit great spatial locality. The tiling technique loads the tiles from global memory into in-block shared memory and threads within a block will compute the tile in the same phase and then moves to the next phase to compute the next tile, as in the following matrix multiplication example.

% data reuse

\subsection{Motivation Summary}

Through reviewing previous work on SpMMul kernel design in Table~\ref{tab:opt}, we find that both improvement and degradation is observed from applying the same technique on different matrices or hardware. Thus, the static optimization cannot always lead to performance improvement, motivating our later designs in the following sections.

% Table generated by Excel2LaTeX from sheet 'Sheet1'

  

%\begin{table}[!h]
%    \caption{Review of Optimizations for SpMMul}
%    \centering
%    \small
%    \begin{tabular}{c|c|c|c|c}
%        \hline
%        Reference & shared memory & thread coarsening & vector loading & sparse matrix tiling \\
%        \hline 
%        \cite{hong2018efficient} & yes & & yes & yes \\
%        \cite{aspt}, \cite{jiang2020novel} & yes & yes & & yes \\
%        \cite{gespmm} & yes & yes & & \\
%        \cite{sputnik}, \cite{wang2020sparsert} & yes & yes & yes &  \\
%        \hline
%    \end{tabular}
%\end{table}

%\begin{table}[h]
%    \caption{Controlled Experiment on Effects of SpMMul Optimizations (Min.-Average-Max.)}
%    \centering 
%    \small 
%    \begin{tabular}{c|c|c|c}
%        \hline
%        Optimization & V100 & RTX2080 & RTX3090  \\ \hline
%        shared memory & 1.03-1.13-1.36 & 1.09-1.32-2.02 & 0.96-1.20-1.68 \\ \hline
%        thread coarsening & 0.75-0.94-1.20 & 0.61-1.20-1.50 & 0.82-0.98-1.25 \\ \hline
%        vector loading & 0.92-1.44-1.77 & 1.41-1.72-1.93 & 1.09-1.55-2.15 \\ \hline
%        sparse matrix tiling* & 0.67-0.91-1.01 & 0.63-0.92-1.06 & 0.54-0.86-1.00 \\ \hline
%        
%        \multicolumn{4}{l}{*Use synthesized block-sparse matrices. Others use R-MAT matrices.}\\
%        
%    \end{tabular}
%\end{table}

==> DAC 2022 - SpMM (arXiv) (1)/data/benchmark.tex <==


\section{Performance Analysis}\label{sec:benchmark}

In this section, we analyze how hardware parameters and data features affect the performance of different designs.


\begin{figure*}[!tp]
    \centering
    \includegraphics[width=\textwidth]{figure/classification.pdf}
    \vspace{-15pt}
    \caption{Importance of features (x-axis) to distinguish different designs. (a) RB and EB. (b) RM and CM. (c) SR and PR.}
    %\vspace{-15pt}
    \label{fig:classification}
\end{figure*}


\subsection{Visualization of Feature Importance}

To provide more insight on how input dynamics affect the performance, we train a variety of binary classification models using the same LightGBM method introduced in Section~\ref{sec:kernel}. Each binary classification problem is defined to classify two design choices in a dimension (\textit{i.e.,} RB/EB, RM/CM, SR/PR). The LightGBM model provides the importance metric to identify the importance of an input feature on the classification results. Thus, we train 4 binary classification models to select the better design for each dimension on one GPU ($3\times 4=12$ models for each dimension in total), with the importance of input features, shown in Figure~\ref{fig:classification}. 

\subsection{Analysis}

\subsubsection{RB and EB.} We can see in Figure~\ref{fig:classification}(a), \textit{std\_row} is the major factor to distinguish these two methods. We have analyzed in Section~\ref{sec:designspace:mloop} and Figure~\ref{fig:rb-eb}, a larger \textit{std\_row} leads to more imbalanced workloads among GPU workers. We show the relationship between \textit{std\_row} and performance ratio of EB/RB in Figure~\ref{fig:stdrow} for all matrices in the SuiteSparse dataset. We can observe a positive correlation in the figure, showing the same conclusion that a larger \textit{std\_row} leads to a higher performance ratio between EB and RB.

\begin{figure}[!tp]
    \centering
    \includegraphics[width=0.48\textwidth]{figure/stdrow-control.pdf}
    \vspace{-15pt}
    \caption{Relationship between \textit{std\_row} and performance ratio of EB/RB. We normalize \textit{std\_row} with average non-zeros in a row. X-axis: normalized \textit{std\_row}. Y-axis: EB/RB.}
    \vspace{-6pt}
    \label{fig:stdrow}
\end{figure}

\subsubsection{RM and CM.} We can see in Figure~\ref{fig:classification}(b) that these two methods cannot be easily distinguished by one certain feature. Features including \textit{std\_row}, \textit{nnz}, and \textit{mat\_size} share similar importance on the classification result. Although we have shown in Figure~\ref{fig:rm-cm}(c) that CM exceeds RM on synthesized matrices with controlled parameters, it hardly achieves better performance against RM on real-world matrices (less than 0.5\% in all scenarios in Figure~\ref{fig:ratio}). Thus, the importance of features in Figure~\ref{fig:classification}(b) is buried by the noise. RM and CM differ in the data access pattern to the dense matrix. Thus, we show the L2 cache hit ratio and the average number of sectors per request (a larger number of sectors means more data is accessed for one time) issues by L2 miss in Figure~\ref{fig:l2} ($N$=32). We show the difference between two groups of matrices (CM is faster than RM, and CM is slower). When CM is faster than RM, it achieves a higher L2 cache hit ratio. Moreover, due to coalesced loading, RM always has a larger number of sectors per request. However, when CM exceeds RM, the metric is improved by 11\% to 26\% for CM, while the difference between two RM groups is only 3\% to 5\%. Thus, CM achieves better performance when the memory access pattern is more coalesced.

\begin{figure}[!tp]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/L2.pdf}
    \vspace{-5pt}
    \caption{Difference between two groups of matrices (CM faster than RM and CM slower than RM) on L2 cache metrics.}
    \vspace{-6pt}
    \label{fig:l2}
\end{figure}


\subsubsection{SR and PR.} We can see in Figure~\ref{fig:classification}(c), \textit{nnz} is the main factor to distinguish these two methods, which is also coordinated with our previous analysis in Section~\ref{sec:designspace:kloop} and Figure~\ref{fig:sr-pr}(c). When \textit{nnz} becomes larger, higher parallelism is required from the hardware perspective. To show how hardware parallelism affects the performance, we use NVIDIA CUDA MPS (Multi-Process Service)~\cite{nvidia2019mps} to set the percentage of CUDA cores when running an algorithm. The result is shown in Figure~\ref{fig:mps}, we run 4 algorithms and normalize the performance to using 10\% CUDA cores. Two RB algorithms achieve a higher performance improvement against two SR methods. The conclusion is aligned with our previous analysis, that PR benefits more from a higher GPU parallelism.
% A larger \textit{nnz} requires higher parallelism, and we further show the relationship between \textit{nnz} and the performance ratio of PR/SR in Figure~\ref{fig:stdrow} for all matrices in the SuiteSparse dataset. We can observe a negative correlation in the figure, showing the same conclusion that a larger \textit{nnz} leads to a better SR performance against PR.

% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figure/nnz-control.pdf}
%     \vspace{-15pt}
%     \caption{Relationship between \textit{nnz} and performance ratio of PR/SR. We normalize \textit{nnz} with the maximum non-zeros in a row. X-axis: normalized \textit{nnz}. Y-axis: PR/SR.}
%     \vspace{-5pt}
%     \label{fig:nnz}
% \end{figure}

%On the other hand, when \textit{nnz} becomes larger, the problem requires higher parallelism from the hardware perspective. To show how hardware parallelism affects the performance, we use NVIDIA CUDA MPS (Multi-Process Service)~\cite{nvidia2019mps} to set the percentage of CUDA cores when running a kernel. The result is shown in Figure~\ref{fig:mps}, we run 4 kernels and normalize the result to the performance of using 10\% CUDA cores. Two kernels based on RB achieve a higher performance improvement compared with two SR methods. The conclusion is aligned with our previous analysis, that PR benefits more from a higher GPU parallelism.




%\subsection{\todo{Benchmarks from hardware perspective}}






% In order to evaluate the performance of the SpMMul design, an unbiased and objective benchmark for the SpMMul problems is required. We present the methodology to design an unbiased and objective benchmark for SpMMul in both general-purpose and domain-specific scenarios.

% \subsection{General-Purpose Scenarios}\label{sec:benchmark:general}

% We implement SpMMul with different selects proposed in Section~\ref{sec:designspace}, and we get 8 static designs. According to the analysis in Section~\ref{sec:designspace:designspace}, one static design cannot always achieve the best performance for different input data. We show the performance of these 8 static designs in Figure~\ref{fig:order} (a)-(c), the detailed setup is in Section~\ref{sec:exp:setup}. The performance of each design is normalized to the best design and we sort the dataset for each design in Figure~\ref{fig:order}.

% Besides the conclusion that the performance is related to the input data characteristics, we can see a severe bias in the benchmark. As we can see in Figure~\ref{fig:order} (d)-(f), the RB+RM+SR design achieves the best performance in most cases, and four designs based on CM hardly win (according to our results, four CM-based designs only win on 0.23\% of all datasets.), this means that CM-based designs do not apply to natural sparse matrices (matrices in SuiteSparse~\cite{davis2011university} are from various domains) rather than synthesized matrices (e.g., matrices used in the controlled experiments in Section~\ref{sec:designspace:nloop}). However, for the other four designs based on RM, an unbiased benchmark for the general-purpose SpMMul should be balance for these designs. 

% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figure/order.pdf}
%     %\vspace{-20pt}
%     \caption{(a)-(c) Normalized performance to the best of 8 static designs proposed in Section~\ref{sec:designspace}. X-axis: different datasets after sorting for each implementation. Y-axis: normalized performance. (d)-(f) The percentage of datasets that one static design achieves the best performance.}
%     %\vspace{-10pt}
%     \label{fig:order}
%  \end{figure}

% Based on analysis above, we propose our benchmark, SpMBench, for SpMMul problems. SpMBench is consisted of 107 (matrix, $N$) pairs, where matrices are selected from SuiteSparse~\cite{davis2011university} and $N$ varies from 1 to 128. The list of SpMBench is anonymously listed online~\cite{spmbench}. Based on SpMBench, percentages of datasets that one static design achieves the best performance are balanced for the four RM-based designs, shown in Figure~\ref{fig:spmbench}. We also include (matrix, $N$) pairs that CM-based designs achieve the best performance to cover conner cases.

% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figure/spmbench.pdf}
%     %\vspace{-10pt}
%     \caption{The percentage of datasets that one static design achieves the best performance using our SpMBench. The legends are same with Figure~\ref{fig:order}.}
%     %\vspace{0pt}
%     \label{fig:spmbench}
%  \end{figure}



% \subsection{Domain-Specific Scenarios}\label{sec:benchmark:specific}

% The motivation of SpMBench is to cover different cases for SpMMul problems. We need to mention that the listed SpMMul is not the only benchmark for SpMMul problems, while it just targets at eliminating biases in previous datasets used for SpMMul designs. Besides, SpMMul kernels are widely used in many domain-specific scenarios, e.g., Graph Neural Networks (GNNs). In these scenarios, a benchmark for general-purpose SpMMul problems is not suitable. Previous works~\cite{gespmm} have mentioned that, GNNs usually use large $N$. GNNs can be used in various domains, e.g., citation networks~\cite{kipf2016semi} and traffic networks~\cite{yu2017spatio}. However, data in different domains show various characteristics which may lead to different performance on different designs. In order to test the performance of SpMMul design for a specific scenario, characteristics from a domain should be analyzed. We have shown in Figure~\ref{fig:order} that CM-based design cannot achieve better performance on natural graphs, thus we plot the performance comparison on other two dimensions in Figure~\ref{fig:gnnbenchmark}.

% We label matrices from three typical domains, including citation networks~\cite{SNAP}, traffic networks~\cite{SNAP}, and matrices in the control problems~\cite{VDOL}. As we can see, matrices from different domains lie in different area. Thus, we can use the coordinates to represent the performance characteristic of a matrix, and generate a performance benchmark for a specific domain by selecting neighbor matrices on the coordinate plain. For example, we only show 4 traffic network matrices, while we can get more matrices from other domains as the benchmark to test the performance of GNN systems on the traffic networks.

% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figure/gnnbenchmark.pdf}
%     %\vspace{-10pt}
%     \caption{Performance characteristics of matrices from different domains.}
%     %\vspace{-10pt}
%     \label{fig:gnnbenchmark}
%  \end{figure}



==> DAC 2022 - SpMM (arXiv) (1)/data/conclusion.tex <==
\section{Conclusions}\label{sec:conclusion}

In this paper, we present a thorough study of Sparse Matrix-Matrix multiplication (SpMM) on GPUs. We consider the SpMM acceleration problem from a novel auto-tuning perspective to be adaptive to input dynamics. We first propose a novel three-loop model with orthogonal design principles specially for sparse problems. We also propose several techniques to implement new designs which are not previously studied. We further propose \kernelname to adaptively optimize code and achieve a better performance considering input dynamics. Evaluations show that \kernelname is the fastest among commercial and academic designs: DA-SpMM achieves an average of \textbf{1.26$\times$}$\sim$\textbf{1.37$\times$} speedup compared with the best NVIDIA cuSPARSE algorithm, and brings up to \textbf{5.59$\times$} end-to-end speedup to applications like Graph Neural Networks. Our methodology of composing design principles into an algorithm space and using heuristic models for algorithm selection can be extended to further studies on sparse acceleration problems.

\begin{figure}[!tp]
    \centering
    \vspace{-5pt}
    \includegraphics[width=0.48\textwidth]{figure/gcn.pdf}
    \caption{Performance comparison for GNNs. X-axis: feature length. Y-axis: Normalized speedup (to the original framework using cuSPARSE). (a) GCN. (b) GraphSAGE.}
    \label{fig:gnn}
 \end{figure}



% \subsection{Data Format} \label{sec:designspace:dfg}

% %The whole dataflow of the SpMMul problem is detailed in Section~\ref{sec:baseline:definition} and pictured in Figure~\ref{fig:overall}. Such an abstract representation is independent from kernel implementation (e.g., usingshared memory, vectorization, coarsening). It also abstracts away the sparse format. The only requirement is that the sparse elements can be retrieved by its row indices, which is straightforward under CSR or any row-first-packing format. We focus on implementations with CSR and row-first-packing COO in the rest of this paper, but present the symmetry in dataflow for row- and column-first-packing scenarios (i.e. CSR and CSC format) in Sec.~\ref{sec-designspace-unify} to illustrate the generality of our design.

% For the format of sparse matrices, CSR is the most common used format in previous designs (e.g., GE-SpMM~\cite{gespmm}, GraphBLAST~\cite{graphblast}, and etc.). Moreover, several frameworks for Graph Neural Networks usually take more than one format to store the sparse matrix. For example, frameworks like DGL~\cite{dgl} and CogDL~\cite{cogdl} take the CSR format for the forwarding while the CSC format for the backpropagation. For the COO format, edges are usually sorted according to their source or destination vertices, leading to similar dataflow of CSR or CSC. By storing sparse matrices with different formats, each kernel design can choose the most suitable format during runtime. Thus, we use the widely-adopted CSR format as default in our latter discussion, unless specifically mentioned.

% \begin{figure}[h]
%     \centering 
%     \includegraphics[width=\linewidth]{figure/unify_dataflow.pdf}
%     \caption{Generalization of the Design Space to Different Dataflows}
% \end{figure}

% \subsection{Generalization to Different Dataflow} \label{sec-designspace-unify}

% All previous discussion is based on the inner-product dataflow. In this subsection, we will show that our dataflow abstraction and definition of design space is general, by re-interpreting it for the outer-product dataflow.



% The outer-product dataflow of an SpMM executes as follows: for each column $k$ of the sparse matrix, first fetch the $k$-th row of the dense input $X_{k,:}$. Next, retrieve the sparse elements $A_{ik}$ from the compressed data structure, use each $A_{ik}$ to multiply the loaded input vector, and scatter-add them to the $i$-th row of the output matrix $Y_{i,:}$. Fig.~\ref{} demonstrates the symmetry between the inner-product and outer-product dataflow. They both have three groups of data, i.e., one dense vector (output/input in the inner-/outer-product), associated with a group of sparse elements (in one row/column), and a group of dense vectors pointed by the indices of the sparse elements (input/output). Note that in this abstraction, the gather-multiply in the inner-product dataflow is symmetric to the scatter-add in the outer-product dataflow. However, in practice, the scatter-add operation involves atomic addition, and have more cost than the gather-multiply. The outer-product dataflow is more challenging to be implemented on GPUs only due to this architectural asymmetry. That is why we only use CSR-based, inner-product dataflow in our experiments. However, all the aforementioned design space apply well to the outer-product dataflow, thanks to the dataflow symmetry.

% By extending the outer-product dataflow, we actually also extend our proposed design space to the SpMM where the sparse matrix is the rhs-matrix. In fact, computing $XA$ is identical to $(A^TX^T)^T$. Since the inner-product and outer-product dataflow can be implemented on the row-major and column-major compressed sparse matrix, and the layout change of the dense matrix can also be interpreted as transposition, our design space covers the design points for $XA$. 

% In summary, in this section, we propose an abstract dataflow and design space for all kinds of SpMV/SpMM.

% % We need to present a the pseudo-code of the baseline design, and I want to show the differences by adopting design 1 to 3 in this section.

% % This section should give hints on why different designs lead to different performance (e.g., element-balancing and row-balancing with std(nnz))


% % \subsection{Applications based on SpMMul}

% % GE-SpMM SpMMul application in GNN,
% % \cite{hu2020featgraph} 
% % \cite{sputnik,wang2020sparsert, bisson2019gpu} : SpMMul applications in sparse NN acceleration. 

% % As two typical sparse kernels in linear algebra, SpMV and SpMM are widely used in various applications. For example, in scientific computing, SpMV is a key primitive in solving large-scale sparse linear systems. In graph analytics, SpMV plays an important role in the propagation and reduction of contributions in the PageRank algorithm~\cite{pagerank}. 

% % Although SpMM could be interpreted as an extension from SpMV considering the new feature dimension in dense tensor, the applications for SpMM are far different from those for SpMV. In Graph Neural Networks, each vertex in the graph is associated with a feature vector. SpMM operation corresponds to copying features of vertexes and aggregating them by taking the sum. GE-SpMM~\cite{gespmm} implements its method in . In sparse transformer, SpMM could be applied in the matrix multiply of masked output of $QK^T$(sparse) and $V$(dense).~\cite{Attention}

% % $$ Attention = Softmax(\frac{QK^T \odot Mask}{\sqrt{d_k}}) V $$

% % In some CNN networks such as MobileNetV1 which have pruned convolution, the $1\times1$ convolution could be computed as SpMM to accelerate the model.~\cite{sputnik}

%\subsection{Conclusion}


==> DAC 2022 - SpMM (arXiv) (1)/data/designspace.tex <==

\begin{figure}[!tp]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/loop.pdf}
    \caption{An overview of the SpMM. (a) Pseudo-code of SpMM with 3 loops. (b) Define SpMM as $A_{M\times K} \cdot X_{K\times N} = Y_{M\times N}$.  (c) $M$-loop: Traversing rows of $A$. (d) $N$-loop: Traversing columns of $X$. (e) $K$-loop: Traversing non-zeros in $A$ and corresponding elements in $X$.}
    \label{fig:overall}
\end{figure}

\section{Design Principles for SpMM on GPUs} \label{sec:designspace}

%This section introduces the algorithm space for SpMMul on GPUs from a novel three-loop perspective. The space is composed of three dimensions, which stem from the input dynamics of SpMMul design. We also propose corresponding optimization techniques for each dimension, and conclude previous designs in this space.

%\begin{figure}[h]
%    \centering 
%    \subfloat[\label{fig-dataflow}]{
%        \includegraphics[width=0.8\linewidth]{figure/dataflow.pdf}
%    }\\
%    \subfloat[\label{fig-design1}]{
%        \includegraphics[width=0.8\linewidth]{figure/designspace_1_balance.pdf}
%    }\\
%    \subfloat[\label{fig-design2}]{
%        \includegraphics[width=0.8\linewidth]{figure/designspace_2_vectorize.pdf}
%    }\\
%    \subfloat[\label{fig-design3}]{
%        \includegraphics[width=0.8\linewidth]{figure/designspace_3_layout.pdf}
%    }
%    \caption{Dataflow Graph and Design Space of SpMV/SpMM}
%\end{figure}

% This section introduces three new dimensions of the design space, that have not been summarized in previous work, but covers the input-dependent features of SpMV/SpMM design and we believe are what distinguishes SpMV/SpMM from dense workload on throughput-oriented architectures like GPUs. For each design dimension proposed, we first explain the design choice and show quantification on the SuiteSparse dataset that prove the feature does span a design dimension, i.e. reveals input-dependent trade-offs.

\subsection{Three-Loop for SpMM} \label{sec:designspace:designspace}

We explore the SpMM problem by digging into three loops of the typical SpMM implementation shown in Figure~\ref{fig:overall}(a). In general, we do not introduce detailed concepts of GPUs when explaining three loops. We use the concept of \textbf{worker} to represent parallel processing units (e.g., threads, warps, and etc.) on GPUs.


\begin{figure*}[!tp]
    \centering
    \begin{minipage}[t]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rb-eb.pdf}
        \caption{$M$-loop. (a) Row Balance (RB): assigning a row to a worker. (b) Element Balance (EB): assigning a given number of elements to a worker.}
        \label{fig:rb-eb}
    \end{minipage}
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/blank.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/rm-cm.pdf}
        \caption{$N$-loop. (a) Row Major (RM): storing $X$ in the row-oriented order. (b) Column Major (CM): storing $X$ in the column-oriented order.}
        \label{fig:rm-cm}
    \end{minipage}
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/blank.pdf}
    \end{minipage}
    \begin{minipage}[t]{0.31\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/sr-pr.pdf}
        \caption{$K$-loop. (a) Sequential Reduction (SR): adding products sequentially.}
        \label{fig:sr-pr}
    \end{minipage}
    \end{figure*}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figure/rb-eb.pdf}
%     \vspace{-5pt}
%     \caption{Different design choices for the $M$-loop. (a) Row Balance (RB): assigning a row to a worker. (b) Element Balance (EB): assigning a given number of elements to a worker.}
%     \vspace{-5pt}
%     \label{fig:rb-eb}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figure/rb-eb-exp.pdf}
%     \vspace{-5pt}
%     \caption{Performance comparison between RB and EB. The EB method achieves better performance when non-zeros in different rows of the sparse matrix become more imbalance.}
%     \vspace{-5pt}
%     \label{fig:rb-eb-exp}
% \end{figure}

\subsection{$M$-Loop: Workload Balance} \label{sec:designspace:mloop}

\textbf{Intuition.} Consider the first loop, $M$-Loop, of SpMM shown in Figure~\ref{fig:overall}(a). $M$-Loop iterates over the rows of the sparse matrix $A$. For each row, the task is to multiply the non-zero elements with the dense elements they point to and accumulate results. If the $m$-th row contains $K_{(m)}$ non-zeros, $K_{(m)} \cdot N$ multiply-add operations are involved. The workload is thus specified for a given $m$ in $1 \sim M$.

\textbf{Design M1: Row Balance (RB).} A simple way for $M$-Loop unrolling and parallel worker assignment is to assign a given number of rows to a worker, which is commonly used in dense problems. Figure~\ref{fig:rb-eb}(a) shows a simple example of the RB method by assigning one row to a worker. By adopting this RB method, we can easily get the row index of each non-zero referring to the worker index. However, workloads of different workers are imbalanced because non-zeros vary in different rows.

\textbf{Design M2: Element Balance (EB).} Another way to unroll $M$-Loop is the fine-grained parallelism by assigning a given number of non-zeros in the sparse matrix $A$ to a worker, which is specially for sparse problems. Figure~\ref{fig:rb-eb}(b) shows an example of the EB method by evenly distributing non-zeros to different workers, where workloads are balanced. However, such a method introduces extra overheads including calculating the row index for a non-zero and partial sum aggregation among different workers in a row.

\textbf{Analysis.} Compared with the RB method, the EB method balances workloads by introducing extra calculations during runtime. Thus, the RB method is supposed to achieve a better performance when the number of non-zeros in different rows is balanced. On the contrary, the EB method tends to be used when workloads become more imbalanced. We later show the controlled experiment on how workload balance affects the choice of RB and EB in Section~\ref{sec:control}.%Obviously, the workload is related to the number of non-zeros in different rows, thus we can use the standard deviation of non-zeros of rows to represent the extent of imbalance.



% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figure/rm-cm.pdf}
%     \vspace{-5pt}
%     \caption{Different design choices for the $N$-loop. (a) Row Major (RM): storing $N$ row by row. (b) Column Major (CM): storing $N$ column by column.}
%     \vspace{-5pt}
%     \label{fig:rm-cm}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figure/rm-cm-exp.pdf}
%     \vspace{-5pt}
%     \caption{Performance comparison between RM and CM. RM achieves better performance when $N$ (width of the dense matrix) becomes larger because of benefits of coalesced loading.}
%     \vspace{-5pt}
%     \label{fig:rm-cm-exp}
% \end{figure}

\subsection{$N$-Loop: Dense Matrix Access Pattern}\label{sec:designspace:nloop}

\textbf{Intuition.} $N$-Loop iterates over the columns of the dense matrix $X$. Different workers process different columns of $X$ according to sparse elements in a given row of $A$ when $m$ is specified in Section~\ref{sec:designspace:mloop}. Note that workers access specific rows in parallel, thus the bandwidth efficiency caused by the memory access pattern is related to the data layout of the dense matrix $X$.

\textbf{Design N1: Row Major (RM).} We first consider the situation to store the dense matrix in a Row Major (RM) way, elements in a row of $X$ are stored in the contiguous memory space. Because different workers process the same rows (shown in Figure~\ref{fig:overall}), the RM layout leads to coalesced memory access pattern~\cite{gespmm}. However, such a data layout suffers from the poor locality for one worker because several rows are skipped, shown in Figure~\ref{fig:rm-cm}(a).


\textbf{Design N2: Column Major (CM).} Another data layout is to store $X$ using a Column Major (CM) order, shown in Figure~\ref{fig:rm-cm}(b). Compared with the RM layout, less memory space is skipped for a worker when processing two neighbor non-zeros in a column, which is beneficial to locality. However, parallel workers cannot benefit from coalesced memory access patterns because data in a row are not stored contiguously, shown in Figure~\ref{fig:rm-cm}(b).

\textbf{Analysis.} Note that the initial and final layout need to be aligned to the previous and next kernel in the application, thus often fixed, we have control on the intermediate matrix layout. When $N$ is small, the RM layout suffers from poor locality because several rows are skipped, while the CM major benefits from locality if the non-zero coordinates $k$'s appear close to each other. However, when $N$ is large, the RM layout shows advantage over CM because it exploits coalesced loading of a row of $X$, which increases the amount of effective data per request and improves bandwidth efficiency. We can easily infer that the parameter $N$ affects the performance of RM and CM for specific sparse matrices. We also show the controlled experiment on the choice of RM and CM in Section~\ref{sec:control}. %and tends to be better when the expected length of skipped elements in CM exceeds a physical threshold (e.g., cacheline size). We can easily infer that the expected length of skipped elements is related to the sparsity and row length ($N$) of the dense matrix $X$.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figure/sr-pr.pdf}
%     \vspace{-5pt}
%     \caption{Different design choices for the $K$-loop. (a) Sequential Reduction (SR): sequentially adding each product. (b) Parallel Reduction (PR): adding each product in parallel with primitives (e.g., warp reduction). (c) Schematic diagram of PR.}
%     \vspace{-5pt}
%     \label{fig:sr-pr}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figure/sr-pr-exp.pdf}
%     \vspace{-5pt}
%     \caption{Performance comparison between SR and PR. SR achieves better performance when the sparse matrix becomes larger, because it achieves a better utilization of each worker.}
%     \vspace{-5pt}
%     \label{fig:sr-pr-exp}
% \end{figure}


\subsection{$K$-Loop: Parallelism Efficiency} \label{sec:designspace:kloop}

\textbf{Intuition.} At last is the third loop, $K$-Loop. In this loop, non-zero elements of a row in $A$ and corresponding elements of a column in $X$ are traversed to calculate the inner product. Note that this loop requires a reduction operation among element pairs to get the sum, the efficiency of parallel workers is related to the way to implement such a reduction operation.

\textbf{Design K1: Sequential Reduction (SR).} A simple way to implement this reduction operation is to assign one worker to calculate the sum and perform the Sequential Reduction (SR) method, shown in Figure~\ref{fig:sr-pr}(a). The SR method achieves high utilization of workers because each worker is always busy when during reduction, which is often used for computation-bounded dense problems. However, such a method loses the potential parallelism existing in the reduction for sparse problems.% (e.g., parallel reduction shown in Figure~\ref{fig:sr-pr}(d)).

\textbf{Design K2: Parallel Reduction (PR).} Another implementation takes the potential parallelism existing in this reduction operation, as is shown in Figure~\ref{fig:sr-pr}(b). We call this method Parallel Reduction (PR), which has been used for sparse problems like Sparse Matrix-Vector Multiplication problems in~\cite{bell2009implementing}. Compared with SR, PR exploits the potential parallelism in reduction, and a typical implementation of PR is a merge-tree shown in Figure~\ref{fig:sr-pr}(d). However, PR suffers from poor utilization of workers because several workers are idle during the reduction, shown in Figure~\ref{fig:sr-pr}(c).



\textbf{Analysis.} The SR and PR methods show two ways of assigning the $K$-Loop to workers. In Figure~\ref{fig:sr-pr}(c), the PR method achieves higher parallelism while the efficiency/utilization of each parallel worker is lowered. When processing larger matrices, the parallelism lost by SR can be compensated by processing more reduction operations in parallel, and the performance tends to be better than the PR method due to higher utilization. On the contrary, PR tends to be better when processing smaller matrices (or GPUs with higher parallelism). The reason is that SR cannot fully utilize the parallelism provided by the GPU. Thus, the performance comparison between the SR and PR methods is closely related to the data size.

\begin{table}[!bp]
    \centering
    \small
    \caption{Summary of previous works in the algorithm space}
      \begin{tabular}{c|c|c|c|c|c|c|c|c}
      \hline
        $M$-Loop & RB    & RB    & RB    & RB    & EB    & EB    & EB    & EB \\
        $N$-Loop & RM    & RM    & CM    & CM    & RM    & RM    & CM    & CM \\
        $K$-Loop & SR    & PR    & SR    & PR    & SR    & PR    & SR    & PR \\
      \hline
        RowSplit\cite{graphblas} &  \checkmark     &       &       &       &       &       &       &  \\
        MergeSpMM\cite{graphblas} & \checkmark      &       &       &       &       &       &       &  \\
        ASpT\cite{aspt} &       &       &       &       &   \checkmark    &       &       &  \\
        GE-SpMM\cite{gespmm} &  \checkmark     &       &       &       &       &       &       &  \\
      \hline
      Ours &   \checkmark    &  \checkmark     &   \checkmark    &    \checkmark   &   \checkmark    &    \checkmark   &    \checkmark   & \checkmark \\
      \hline
      \end{tabular}%
      %\vspace{-15pt}
    \label{tab:designspacesummary}%
  \end{table}%

%\subsection{Implementations} \label{sec-designspace-impl}


% We also detailed all implementations with optimization methods (e.g., vectorized loading, and etc.) introduced in Section~\ref{sec:baseline} if appliable. 

% \begin{algorithm}[!tp]
%     \caption{Pseudo-code of SpMMul implementations}\label{alg:SpMMul}
%     \begin{algorithmic}[1]
%       \REQUIRE $A$ and $X$
%       \ENSURE $Y = A\cdot X$
%       \FOR {each $warp$ in parallel}
%       \STATE assign rows to $warp$
%       \FOR {each $warp$ with one row ($A[m,:]$) in parallel}
%       \FOR {each $X[:,n]$ in parallel}
%       \STATE load each $X[k,n]$
%       \STATE reduce\_sum ($A[m,k] \times X[k,n]$)
%       \ENDFOR
%       \ENDFOR
%       \ENDFOR
%       \FOR {each $Y[m,:]$ in parallel}
%       \STATE $Y[m,:]$ = atomic\_add (related $warps$)
%       \ENDFOR
%       \RETURN $Y$
%     \end{algorithmic}
%   \end{algorithm}





%   \begin{figure}[!bp]
%       \centering
%       \includegraphics[width=0.48\textwidth]{figure/ratio.pdf}
%       \vspace{-15pt}
%       \caption{Ratio of each design that achieves the best performance on SpMMul ($N$ is from 1 to 128).}
%       \label{fig:ratio}
%   \end{figure}



\subsection{Comparison with Previous Works}

Based on the novel three-loop model, we summarize previous SpMM designs in Table~\ref{tab:designspacesummary}. By decomposing the mathematical formulation of SpMM, combining design principles is capable of covering all previous designs. Moreover, we can also find new designs for the SpMM (\textit{e.g.,} RB+RM+PR.). We implement all 8 designs based on these design principles, which are further used for performance tuning in later sections.


  
  



==> DAC 2022 - SpMM (arXiv) (1)/data/experiment.tex <==


\section{Experimental Results}\label{sec:exp}

\subsection{Experimental Setup}\label{sec:exp:setup}

\subsubsection{Environments.}\label{sec:exp:setup:env}

We use three different GPUs set up our experimental environments for previous and this sections:

NVIDIA \textbf{RTX 3090.} Compute Capability 8.6 (68 Ampere SMs at 1.395 GHz, 24 GB GDDR6x, 936 GB/s bandwidth).%Host CPU: AMD Ryzen Threadripper 3970X (32 cores).

NVIDIA \textbf{RTX 2080.} Compute Capability 7.5 (46 Turing SMs at 1.515 GHz, 8 GB GDDR6, 448 GB/s bandwidth).%Host CPU: Intel Core i7-9700K (8 cores).

NVIDIA \textbf{Tesla V100.} Compute Capability 7.0 (80 Volta SMs at 1.370 GHz, 16 GB HBM2, 900 GB/s bandwidth).%Host CPU: Intel Xeon CPU E5-2698 v4 (20 cores).


\subsubsection{Baselines.}

\textbf{GE-SpMM}~\cite{gespmm} is a state-of-the-art open-source SpMM design on GPUs, it achieves better performance against other open-source design like GraphBLAST~\cite{graphblast}.

\textbf{ASpT}~\cite{aspt} adopts a matrix tiling preprocessing step to process dense and sparse sub-matrix separately during runtime. We only count the execution time of ASpT while excluding the preprocessing time. Moreover, ASpT only supports $N=32$ and $N=128$ cases.

\textbf{NVIDIA cuSPARSE}~\cite{cusparse} is a vendor library by NVIDIA. We use the routine \texttt{cusparseSpMM} for SpMM, we use version 11.2.

All results are normalized to the best cuSPARSE algorithm for each matrix. All codes are compiled using \texttt{nvcc} 11.2 with -\texttt{O3} flag.


\subsubsection{Datasets.}\label{sec:exp:setup:dataset}

We use SuiteSparse collection~\cite{davis2011university} with 956 matrices (We use the script of ASpT~\cite{aspt} to select these matrices which removes isomorphic one to enable diversity) to test performance. 

\subsection{Performance of Heuristic Kernel}

We compare the DA-SpMM design with GE-SpMM~\cite{gespmm}, ASpT~\cite{aspt}, and two cuSPARSE~\cite{cusparse} SpMM algorithms (Alg3 and Alg7 in Figure~\ref{fig:cusparsekernel}, which are two best static algorithms). All results are normalized to the best cuSPARSE SpMM algorithm on each matrix, shown in Figure~\ref{fig:overall-result}. We can get following conclusions:

%\squishlist

    %\item \textbf{Against static cuSPARSE.} For different $N$ from 2 to 128, \kernelname achieves an average speedup of \textbf{2.60$\times$} to \textbf{2.96$\times$}, \textbf{2.42$\times$} to \textbf{2.66$\times$}, \textbf{2.36$\times$} to \textbf{2.57$\times$} on three GPUs, respectively.

    \textbf{Against the static cuSPARSE algorithm.} For different $N$ from 2 to 128, \kernelname achieves an average speedup of up to 2.96$\times$, 2.66$\times$, 2.57$\times$ on three GPUs, respectively.

    \textbf{Against different cuSPARSE algorithms with the best performance on each matrix.} For different $N$ from 2 to 128, DA-SpMM achieves an average speedup of 1.37$\times$, 1.26$\times$, and 1.30$\times$ on three GPUs, respectively. For large $N$ (e.g., $N=128$), \kernelname achieves higher speedup of 1.60$\times$, 1.36$\times$, and 1.30$\times$, respectively. 
    
    \textbf{Against ASpT.} For $N=32$, DA-SpMM achieves an average speedup of 1.14$\times$, 1.14$\times$, and 1.06$\times$, respectively. For $N=128$, the speedup is 1.20$\times$, 1.14$\times$, and 1.05$\times$. The preprocessing time of ASpT is not counted.

    \textbf{Against GE-SpMM.} DA-SpMM achieves significant improvements for small $N$ (4.99$\times$, 5.23$\times$, and 5.40$\times$ for $N=2$). When $N$ becomes larger, the performance of GE-SpMM improves. For $N=128$, the speedup against GE-SpMM is 1.29$\times$, 1.04$\times$, and 1.59$\times$ on three GPUs, respectively. When $N$ becomes larger, DA-SpMM prefers to select RM for $N$-loop and SR for $K$-loop in most cases. These two selections are the same with the design in GE-SpMM, which means that GE-SpMM does reach the optimal design point for these cases, except for the balance design in the $M$-loop.

%\squishend




\subsection{Controlled Experiments}\label{sec:control}

As we have analysed in Section~\ref{sec:designspace}, the choice of different algorithm for each loop depends on input dynamics. Thus, we synthesize matrices and conduct controlled experiments.

\subsubsection{RB-EB} We take three sparse matrices with identical size and sparsity, but different $std\_nnz$, \textit{i.e.,} the standard deviation of the number of non-zeros in each row. The matrices are synthesized R-MAT graphs ~\cite{chakrabarti2004r} by tuning parameters related to element distribution. The result is shown in Figure~\ref{fig:control}(a). The EB method exceeds the RB method as the standard deviation of non-zeros in each row grows, because the imbalance among different workers becomes the main factor for the performance difference.

\subsubsection{RM-CM} We synthesize one same sparse matrix with three different dense matrices, with R-MAT method~\cite{chakrabarti2004r}. We vary $N$ for the dense matrix. The result is shown in Figure~\ref{fig:control}(b). The RM layout achieves higher performance against the CM layout when $N$ gets larger. The reason is that larger $N$ leads to coalesced load for different workers. In contrast, the CM implementation always needs to skip elements in the dense vector, thus the effective data per request is inherently limited.%and worse locality on the column dimension because more elements in a row are skipped.

\subsubsection{SR-PR} We synthesize three matrices with the same sparsity and non-zero distribution, but different non-zeros, with R-MAT method~\cite{chakrabarti2004r}. The bars in Figure~\ref{fig:control}(c) display non-zeros of each matrix, and the lines plot the relative performance of SR against PR. When the matrix is small, the PR method is better than the SR method because it saturates parallelism, but SR gains advantages when the matrix size gets larger because the utilization of one worker becomes the main factor for the performance.

\begin{figure}[!tp]
    \centering
    %\vspace{-10pt}
    \includegraphics[width=0.48\textwidth]{figure/controlexp.pdf}
    \caption{Controlled experiments to show how input data dynamics affect choice of different algorithms for each loop. (a) RB-EB: workload balance. (b) RM-CM: data access pattern. (c) SR-PR: total workloads.}
    \label{fig:control}
 \end{figure}

\subsection{Performance of Heuristic Kernel in GCNs}

We integrate DA-SpMMul into the Graph Neural Network framework, DGL~\cite{dgl}, to compare the end-to-end performance on RTX 3090 with GCN~\cite{kipf2016semi} and GraphSAGE~\cite{graphsage} models. We test the inference speedup with on the Reddit dataset~\cite{reddit}, in Figure~\ref{fig:gnn}. By using DA-SpMM, we achieve up to \textbf{5.59$\times$} and \textbf{5.27$\times$} speedup against the original DGL framework on two GNN models, respectively.



==> DAC 2022 - SpMM (arXiv) (1)/data/heuristickernel.tex <==
\begin{figure}[!tp]
    \centering
    \includegraphics[width=0.48\textwidth]{figure/heuristickernel.pdf}
    \caption{Average normalized performance of the heuristic DA-SpMM kernel. (a) \kernelname based on features of input data against 8 static designs proposed in Section~\ref{sec:designspace}. (b) A unified \kernelname kernel for different GPUs.}
    \label{fig:heuristickernel}
 \end{figure}


\section{Heuristic Kernels}\label{sec:kernel}

\subsection{Heuristic Adaptability}

We get 8 optimized SpMM algorithms in Section~\ref{sec:impl}, and we also analyze that characteristics of the input data affect the performance of implementations. Then, we further test the performance of all these 8 designs on 3 different GPUs with 956 matrices in the SuiteSparse dataset (with detail setups in Section~\ref{sec:exp:setup}). The average normalized performance (the meaning is the same as that in Figure~\ref{fig:cusparsekernel}) is shown in Figure~\ref{fig:heuristickernel}(a). We can get the same conclusion that a single algorithm cannot always achieve the best performance on different input data, and a single algorithm with the best average normalized performance is $<$70\%.

Thus, to be adaptive to input dynamics and achieve a better performance, auto tuning has been proved as an effective method. We leverage the gradient boosting framework LightGBM~\cite{lightgbm} to train a prediction model to select the best design from the 8 different designs. We select a collection of features extracted from both the sparse matrix and the dense matrix as the input vector to our model, as in Table~\ref{tab:feature}.%We also choose hardware features (e.g., size of L2 cache and number of CUDA cores) as input to show how hardware parameters affect the performance.

\begin{table}[!h]
    \centering
    \caption{Extracted features in heuristic kernels.}
    \small
      \begin{tabular}{c|l}
      \hline
      Feature & Meaning \\
      \hline
        \textit{nnz} & Number of non-zeros in the sparse matrix \\
        \textit{mat\_size} & Size of the sparse matrix \\
        \textit{std\_row} & Standard deviation of non-zeros in rows \\
        \textit{N} & Width of the dense matrix \\
      \hline
      \end{tabular}%
    \label{tab:feature}%
  \end{table}%

%The performance is shown in Figure~\ref{fig:ratio}. We can get a similar conclusion as the performance of different cuSPARSE kernels in Figure~\ref{fig:cusparsekernel}, one single implementation cannot achieve the best performance on different datasets.

%Thus, to be adaptive to input dynamics and achieve a better performance, auto tuning has been proved as an effective method. Among auto tuning solutions, Machine Learning (ML) techniques are commonly used for regression and classification problems. Compared with other ML methods, gradient boosting is characterized by synthesizing weak prediction models (usually decision trees), to derive a strong prediction model. 






% \begin{table}[!h]
% %\vspace{-10pt}
% \caption{Extracted features in heuristic kernels.}
% \small
% \centering
% \label{table:feature}
% \begin{tabular}{c|l}
% \hline
% Feature & Meaning \\ \hline
% \textit{nnz} & number of non-zeros in the sparse matrix \\ 
% \textit{mat\_size} & size of the sparse matrix \\ 
% \textit{avg\_row} & average number of non-zeros in rows \\ 
% \textit{avg\_col} & average number of non-zeros in columns \\ 
% \textit{dev\_row} & standard deviation of non-zeros in rows \\ 
% \textit{dev\_col} & standard deviation of non-zeros in columns \\ 
% \textit{N} & width of the dense matrix \\ \hline
% \end{tabular}
% %\vspace{-10pt}
% \end{table}

% Table generated by Excel2LaTeX from sheet 'Sheet1'



\begin{figure*}[!tp]
    \centering
    \includegraphics[width=\textwidth]{figure/overall-result.pdf}
    \caption{SpMM performance comparison among our DA-SpMM, GE-SpMM~\cite{gespmm}, and ASpT~\cite{aspt}, and cuSPARSE~\cite{cusparse}.}
    \label{fig:overall-result}
\end{figure*}
 
\subsection{Evaluation}

\subsubsection{Individual Model.}
We also use the average normalized performance as the criterion to evaluate the performance of our heuristic kernel, \kernelname. Here we train three individual models for each GPU. We set the ratio of train, validation, and test data to 40\%, 10\%, and 50\%, respectively. As is shown in Figure~\ref{fig:heuristickernel}(a), \kernelname achieves \textbf{98.62\%}, \textbf{98.03\%}, and \textbf{98.33\%} normalized performance on 3 GPUs (an average of \textbf{98.33\%}), respectively. In contrast, the best normalized performance of one static design is lower than 70\%.

%Thus, \kernelname solves the problem that the static kernel optimization cannot be adaptive to the input dynamics.

\subsubsection{Unified Model.} We further test the performance of migrating the model trained by one GPU to another, leading to an average of 5.38\% performance loss (\textit{e.g.,} using \kernelname model trained by RTX 2080, \textit{i.e.,} DA-SpMM (RTX 2080), for Tesla V100 degrades the performance from 98.33\% to 90.64\%). To be adaptive to different GPUs, we further distinct different GPUs to train one unified LightGBM model. The result shows that, a unified \kernelname can not only solve the performance loss of migrating the model, it also further achieves the better performance, \textbf{99.50\%}, \textbf{98.13\%}, and \textbf{99.17\%} on 3 GPUs (an average of \textbf{98.93\%}).

\subsection{Heuristic Kernel Conclusion}

By introducing the heuristic model to dynamically select kernels with better performance, \kernelname is adaptive to input dynamics. With only data features for model training, \kernelname improves the normalized performance from less than 70\% to over 98\% for different GPUs. By introducing hardware features, \kernelname further improves the performance with a unified heuristic model.


% \subsubsection{RB and EB}
% As illustrated by figure \ref{fig:classification}(a), the most important features when choosing between RB and EB are N, avg\_row and dev\_row. The insight behind this is that the EB method can achieve better performance when the distribution of non-zero elements in each row is not balanced by introducing extra computation to balance the workload. N influence this design choices because \todo{need a reason}. The features avg\_row and dev\_row influence the choice of RB and EB because they are directly related to the balance of elements in rows.

% \subsubsection{RM and CM}
% The results of RM and CM in figure \ref{fig:classification}(b) can be confusing and hard to explain because it doesn't follow the intuition that $N$ should be of great importance when choosing between RM and CM. This is because the run-time data we obtain from SuiteSparse is biased.  We notice that only under less than 1\% circumstances does CM outperform RM, which makes the model hard to train, which also calls for a more unbiased benchmark. 

% \subsubsection{SR and PR}
% As illustrated by figure \ref{fig:classification}(c), the most important features for SR and PR is $nnz$ and $N$. The insight behind this is that there is a tradeoff between SR and PR. The PR method exploits parallelism in the reduction operation but may suffer from poor utilization of workers because of the idle workers. When the matrix is large, SR outperforms PR due to its high utilization. The feature $nnz$ is closely related to the number of reduction operations in SpMMul and therefore is of great importance when choose between SR and PR. And $N$ \todo{is always important in SpMMul because}


% 3. The importance of different features.
% \par
%     For the sparse matrix, we compress it into a vector by feature extraction. Obviously,  not all the features of the sparse matrix (that is, the dimensions of the “feature vector”) play the same role in the training and prediction procedure. Or rather, some features might just have little to do with computational performance, which implies that then will be given a smaller weight in the heuristic kernel. Considering that they do not play a substantial role in the kernel construction, and some of them can cost a lot to obtain in the preprocessing stage of sparse matrices. Thus, oriented to achieve the balance between the cost of matrix preprocessing and prediction accuracy, we will remove these "secondary" features from the design of the kernel, which won’t lead to prominent deterioration of the kernel’s performance.
% \par
%     Further, about the screening of important features, a typical and strateforward example is that we prefer “row features” (which stands for features associated with rows of the sparse matrix) to “column features”. On the one hand, in the CSV format, because of the “row priority” in storage, the “column features” are more time-consuming to obtain. On the other hand, in SpMV and SpMM, we multiply the rows of sparse matrix to the dense vector/matrix, indicating that the distribution of non-zero elements in the column direction will not have a direct impact on the multiplication process. Actually, with the help of Lightgbm and xgboot classifier, we can evaluate the significance of each feature in the heuristic kernel (shown in Figure 10.).


==> DAC 2022 - SpMM (arXiv) (1)/data/implementation.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.48\textwidth]{figure/impl.pdf}
    \caption{Implementations of different SpMM algorithms under the algorithm space with proposed techniques, number of threads in a warp is 4. (a) An example of SpMM with legends in latter subfigures. (b) Using \texttt{for-loop} to reduce $>4$ elements for RB. (c) Using \texttt{float2/float4} to load multiple dense elements for RM. (d) Using shared memory to cache sparse elements for reuse. (e) Using a prefix sum network with conditional reduction for EB.}
    \label{fig:impl}
\end{figure}

\section{Implementations} \label{sec:impl}

As mentioned in Table~\ref{tab:designspacesummary}, previous studies on SpMM only explore both RB and EB methods for the $M$-Loop, while CM for the $N$-Loop and PR for the $K$-Loop is lacking. Implementing CM is trivial derived from the implementation of the corresponding RM design by storing the dense matrix in a column-oriented order. Thus, we can easily get RB+CM+SR and EB+CM+SR from current implementations.

\textbf{RB+RM+PR}. The main challenges of implementing PR under RB include: (1) The number of elements to perform the reduction may be larger than the number of threads in a GPU warp, thus the reduction cannot be processed within one warp instruction. (2) Different columns require same non-zeros in a row of the sparse matrix, leading to redundant data loading. Figure~\ref{fig:impl}(a) shows an example of performing reduction on 5 sparse rows with 6/2/0/3/1 non-zeros each row, we set the number of threads in a warp to 4. We utilize a \textbf{\texttt{for-loop} (Technique 1)} in Figure~\ref{fig:impl}(b), for the first challenge to enable reduction of $>$4 (number of threads in a warp) elements (\textit{e.g.,} the first row). For the second challenge, we utilize \textbf{\texttt{float2/float4} (Technique 2)}, shown in Figure~\ref{fig:impl}(c), primitive to load multiple elements in consecutive columns in the dense matrix, and these columns are processed by a warp. However, the \texttt{float2/float4} primitive only enables us to process at most 4 columns within a warp. In order to reuse data for large $N$ (columns in the dense matrix), we further utilize \textbf{shared memory (Technique 3)}, shown in Figure~\ref{fig:impl}(d), to cache sparse elements for different columns. Thus, these elements can be reused for multiple columns.

\textbf{EB+RM+PR}. The main challenges of implementing PR under EB include: (1) A warp needs to perform reduction on different rows for the same number of elements in the sparse matrix. (2) The same challenge as the second challenge in RB+RM+PR, thus \textbf{Technique 2/3} can still be used. Inspired by the prefix sum network, we propose the \textbf{conditional reduction (Technique 4)}, shown in Figure~\ref{fig:impl}(e), method to solve the first challenge. Besides the partial reduction result, a thread records a \texttt{index} flag to distinguish the row. For each reduction step, the datapath of the prefix sum network is activated if two threads share the same \texttt{index} flag. The outputs of such a conditional prefix sum network are valid for the first (leftest) thread or the thread with different \texttt{index} compared with the thread on its left. For rows assigned to different warps, an \texttt{atomic\_add} operation is performed get the final reduction result.

\textbf{RB+CM+PR}. The only difference to RB+RM+PR is that the dense matrix is stored in a column-oriented order, thus \textbf{Technique 2} cannot be used because elements in a row are not stored consecutively, while \textbf{Technique 1/3} are applied.

\textbf{EB+CM+PR}. Similar to RB+CM+PR, \textbf{Technique 2} is not applied, while \textbf{Technique 3/4} in EB+RM+PR are used.

%Based on the analysis with the algorithm space above, we get 8 SpMMul designs (i.e., \{RB, EB\} $\times$ \{RM, CM\} $\times$ \{SR, PR\}) on GPUs. In Algorithm~\ref{alg:SpMMul} and Figure~\ref{fig:design-space-implementation}, we detail these 8 designs with GPU kernel implementations. 




% The difference between RB and EB lies in Line 2 and 10-12 in Algorithm~\ref{alg:SpMMul}. For the row assignment (Line 2), RB assigns a row of $A$ to one warp, while EB may assign one row to multiple rows. Thus, EB requires an extra phase to aggregate reduction results from different warps (Line 10-12). The diagram is shown in Figure~\ref{fig:design-space-implementation}(a) and (b). For RB, the workload of $A[1,:]$ and $A[2,:]$ is assigned to two warps individually. However, the workload of $A[1,:]$ is assigned to both warps for EB, and an atomic add operation is required to get $Y[1,:]$.

% Then, we explain the other two loops together from Figure~\ref{fig:design-space-implementation}(c) to (f) to show the memory access pattern and parallelism. The difference between the RM and CM layouts is not explicitly shown in Algorithm~\ref{alg:SpMMul}. However, these two layouts affect the memory access pattern of warps or threads on GPUs. For RM, elements in a row of $X$ are contiguously stored in the GPU memory, thus these elements are coalesced loaded when different warps or threads execute in parallel, shown in Figure~\ref{fig:design-space-implementation}(c) and (e). More specifically, multiple columns can be assigned to a warp for RM+PR design by using vectorization primitives on GPUs (i.e., float2/float4), shown in Figure~\ref{fig:design-space-implementation}(e). For CM, the locality along $K$ dimension is explored because columns are contiguously stored, shown in Figure~\ref{fig:design-space-implementation}(d) and (f).

% The difference between SR and PR lies in Line 6 in Algorithm~\ref{alg:SpMMul}. SR uses one thread in a warp to sequentially get the reduction result between sparse elements of a row of $A$ and a column of $X$, shown in Figure~\ref{fig:design-space-implementation}(c) and (d). On the contrary, PR uses one warp to get the reduction result in parallel with warp reduction primitives, shown in Figure~\ref{fig:design-space-implementation}(e) and (f).

==> DAC 2022 - SpMM (arXiv) (1)/data/introduction.tex <==
\section{Introduction}


\begin{figure}[!bp]
    \centering
    \includegraphics[width=0.48\textwidth]{figure/motivation-cusparse.pdf}
    \caption{The left part shows the average normalized performance of different SpMM algorithms in cuSPARSE~\cite{cusparse} (to the algorithm with the best performance, using the geometric mean on the SuiteSparse~\cite{davis2011university}), $N$ is the width of the dense matrix. The right part shows an example of how the average normalized performance is calculated for 2 matrices.}
    %\vspace{-12pt}
    \label{fig:cusparsekernel}
\end{figure}


Sparsity is a key enabler of future Artificial Intelligence~\cite{low2012distributed, xiao2017tux2, han2015deep}. Sparsity enables fast and energy-efficient training and inference in various domains~\cite{eie, mobilenets, sanh2020movement, fedus2021switch}. However, sparse computation loses to its dense counterpart in terms of throughput, especially on throughput-oriented architectures like GPUs. In many emerging applications such as Graph Neural Networks (GNNs)\cite{gespmm}, recommendation~\cite{Asgari2021FAFNIRAS} and large language models~\cite{wang2019structured}, Sparse Matrix-Matrix Multiplication (SpMM) has served as fundamental components and dominated total execution time~\cite{gespmm, eie}. SpMM can be formulated by the multiplication between a sparse matrix and a dense matrix, exposing high potential parallelism and requires high throughput, thus many previous studies focus on accelerating SpMM using GPUs~\cite{aspt, jiang2020novel, gespmm, sputnik, wang2020sparsert}.



% (1) TACO
% (2) Nisa
% (3) graphblast, ge-spmm

% \begin{table}[!h]
%     \centering
%     \footnotesize
%     \vspace{-13pt}
%     \caption{Normalized SpMM performance of different kernels (Alg0$\sim$Alg9) in cuSPARSE (to the kernel with the best performance, using geometric mean on the SuiteSparse~\cite{davis2011university} dataset), $N$ is the width of the dense matrix.}
%     \vspace{-5pt}
%       \begin{tabular}{c|r|r|r|r|r|r}
%       \hline
%       \multirow{2}[4]{*}{} & \multicolumn{2}{c|}{RTX 3090} & \multicolumn{2}{c|}{RTX 2080} & \multicolumn{2}{c}{Tesla V100} \\
%   \cline{2-7}          & \multicolumn{1}{c|}{$N=8$} & \multicolumn{1}{c|}{$N=32$} & \multicolumn{1}{c|}{$N=8$} & \multicolumn{1}{c|}{$N=32$} & \multicolumn{1}{c|}{$N=8$} & \multicolumn{1}{c}{$N=32$} \\
%       \hline
%       Alg0  & 34.1\% & \textbf{79.7\%} & 35.1\% & 77.6\% & 33.1\% & 74.1\% \\
%       Alg1  & 33.5\% & 77.7\% & 34.9\% & 77.0\% & 33.2\% & 74.2\% \\
%       Alg2  & 32.9\% & 76.7\% & 34.7\% & \textbf{78.2\%} & 36.7\% & 79.9\% \\
%       Alg3  & 32.9\% & 76.4\% & 34.7\% & 78.1\% & 36.8\% & \textbf{80.0\%} \\
%       Alg4  & 63.0\% & 42.2\% & 69.1\% & 49.0\% & 61.3\% & 43.7\% \\
%       Alg5  & 62.6\% & 42.1\% & 68.8\% & 48.8\% & 61.3\% & 43.8\% \\
%       Alg6  & \textbf{73.3\%} & 51.4\% & 72.6\% & 46.9\% & 74.9\% & 52.7\% \\
%       Alg7  & 72.9\% & 45.6\% & \textbf{76.7\%} & 47.1\% & \textbf{80.0\%} & 49.6\% \\
%       Alg8  & 19.6\% & 12.5\% & 21.5\% & 14.9\% & 23.3\% & 14.9\% \\
%       Alg9  & 60.0\% & 42.1\% & 61.0\% & 40.7\% & 58.0\% & 40.7\% \\
%       \hline
%       \end{tabular}%
%       \vspace{-10pt}
%     \label{tab:cusparsekernel}%
%   \end{table}%

%\footnote{CSR + ROW\_MAJOR + CUSPARSE\_SPMM\_ALG\_DEFAULT}


However, improving the performance of SpMM suffers from the challenge of handling the input dynamics, \textit{i.e.,} the performance is dependent on not only the static code optimizations, but also the dynamic input characteristics. We test the performance of 10 SpMM algorithms in NVIDIA cuSPARSE~\cite{cusparse} on different sparse matrices (956 matrices in the SuiteSparse~\cite{davis2011university} dataset) and different width of the dense matrix ($N=8$ and $N=32$). Figure~\ref{fig:cusparsekernel} shows performances of ten algorithms normalized to the best algorithm for each matrix. A single algorithm cannot always achieve the best performance on different input data, and the maximum performance loss with a single algorithm is >85\% (\textit{e.g.,} Alg8, $N=32$ on RTX 3090). Despite its importance and obvious difficulty, tackling input dynamics is missing from the focus of previous work. For example, GE-SpMM~\cite{gespmm} adopts techniques like thread coarsening and shared memory to optimize the performance when $N$ is large. However, GE-SpMM is slower than cuSPARSE when $N$ is small (e.g., running GraphSAGE~\cite{graphsage}, $N$=16, in GE-SpMM's paper). Another example is that the thread coarsening technique cannot always achieve benefit on different data (Figure 8 in GE-SpMM's paper).% (guyue): I think we need more example, simple statements


% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=0.25\textwidth]{figure/motivation-new.pdf}
%     \vspace{-15pt}
%     \caption{The scope of this work on SpMM problems compared with previous works~(e.g., TACO~\cite{taco}, Nisa \textit{et al.}~\cite{Nisa2018}, GE-SpMM~\cite{gespmm}, GraphBLAST~\cite{graphblast}). We introduce a novel design space for SpMM and an ML-based heuristic method to maximize the kernel performance of SpMM on GPUs.}
%     \vspace{-25pt}
%     \label{fig:motivation}
% \end{figure}

Observing that previous work limits their optimizations to some specific scenarios, we ask this question: how can we design a \textit{generally good} SpMM kernel for all kinds of scenarios? Our answer is that not a single design, but the \textit{careful composition and adaptive usage} of many designs, can well address input dynamics. Previous work has proposed many ad-hoc optimizations with limited rule-based selection models. In this paper, we seek to propose design-composition-guided new optimizations, and use data-driven ML models to make input-dynamic choices of implementations. We also solve the following challenges:
%\dl{Thus, to overcome the shortcoming that a single algorithm or specific optimizations cannot be adaptive to input dynamics, we consider the SpMM acceleration problem from a novel auto tuning perspective~\cite{chen2018tvm, graphit}. However, introducing auto tuning for SpMM needs to solve following challenges:}
\textbf{(1) Orthogonal design principles considering sparsity.} Optimizations in dense problems consider little of sparsity in SpMM. We need to extract orthogonal design principles considering sparsity to form algorithms for auto tuning. \textbf{(2) Nontrivial implementations in the algorithm space.} Combining techniques (\textit{e.g.,} workload balance for unbalanced matrices~\cite{graphblas} and parallel reduction to utilize idle GPU threads~\cite{bell2009implementing}) can bring benefits to specific inputs, while implementing them is nontrivial and missed in previous studies. \textbf{(3) Heuristic adaptability to input dynamics.} An efficient heuristic model is required to be adaptive to input dynamics. We make following contributions in this paper:


%Thus, to optimize SpMMul performance with the auto tuning method, modeling a complete design space for SpMMul on GPUs is required. However, such a problem is rarely analyzed in previous studies. We formulate the SpMMul problem into a complete design space with three dimensions constructed by three loops in this paper. To evaluate the performance of an SpMMul kernel design on GPUs, an unbiased and objective benchmark is required. However, previous studies use general-purpose sparse matrix benchmarks. These benchmarks are not specifically designed for SpMMul, leading to unfairness and bias for performance comparison. By modeling the complete design space, we illustrate whether a sparse matrix or graph benchmark covers all cases. Then, an objective benchmark is given in this paper. Based on these analyses, we further propose our heuristic SpMMul kernel design on GPUs with auto tuning in the proposed design space. 

%in Sparse Matrix-Vector Product (SpMV), which elements in the input vector are loaded is dependent on where the non-zeros appear in the sparse matrix, making it hard to optimize memory access pattern. Tiling, an effective optimization to improve data reuse, is also difficult to apply because we cannot forsee the spatially clustered non-zeros. 

%Other than heuristic optimization, auto tuning is an effective technique in kernel optimization.  For a design space to be practical, compiler designers always exploit from prior experiences to prune a potentially huge design space. For tensor computation, it can be tiling, fusion, parallelism. For graph analytics, it can be the propagation direction (push/pull), the graph partition. In this paper, we make our attempt to picture the design space of two important sparse matrix primitives, names SpMV and SpMM, on throughput-oriented architectures like GPUs. 




\squishlist

    \item \modified{\textbf{We propose three sparsity-unique design principles for SpMM on GPUs.} We decompose the mathematical formulation of the SpMM, with orthogonal design principles specially for sparse problems. We propose 8 algorithms according to 3 dimensions in the space, which not only cover previous designs, but also come up with new designs which are not studied.}
    
    \item \textbf{We propose nontrivial techniques to complete the algorithm space.} We propose several techniques complete missing algorithms in the space. For example, we introduce the conditional reduction to implement workload balance for imbalance matrices and parallel reduction to utilize idle GPU threads.
    
    \item \textbf{We design a data-aware kernel, \kernelname, to be adaptive to input dynamics.} \kernelname considers input dynamics, and dynamically selects a design with better performance for SpMM. \kernelname improves the performance of a static design from $<$70\% to $>$98\% (normalized to the best design on each dataset).
    
\squishend



DA-SpMM achieves \textbf{1.26$\times$}$\sim$\textbf{1.37$\times$} speedup on average compared with the best NVIDIA cuSPARSE algorithm, and brings up to \textbf{5.59$\times$} end-to-end speedup to applications like Graph Neural Networks.



%The following of this paper is organized as: Section~\ref{sec:relatedwork} introduces related works. Our three-dimension algorithm space with optimizations is shown in Section~\ref{sec:designspace}. Techniques for miss algorithm implementation are introduced in Section~\ref{sec:impl}. Our heuristic SpMM kernel, \kernelname, is detailed in Section~\ref{sec:kernel}. Extensive experimental results are shown in Section~\ref{sec:exp}. Section~\ref{sec:conclusion} concludes this paper.



==> data/baseline.tex <==


\section{Motivation}\label{sec:baseline}


This section introduces the definition with a conceptual dataflow for SpMMul. Then, we conduct a comprehensive study on previous SpMMul optimizations with thorough controlled experiments, showing that previous SpMMul techniques do suffer from input dynamics.

\subsection{SpMMul Definition}\label{sec:baseline:definition}

Both SpMV and SpMM can be unified with Equation~(\ref{equ:Y=AX}):

\vspace{-5pt}
\begin{equation}\label{equ:Y=AX}
    A_{M\times K} \cdot X_{K\times N} = Y_{M\times N}
\end{equation}

A sparse matrix $A_{M\times K}$ is multiplied by a dense matrix $X_{K\times N}$ to form a dense output matrix $Y_{M\times N}$. Specifically, we have $N=1$ for SpMV, and $N>1$ for SpMM. Previous studies show that, SpMMul is one of the most used and time-consuming operations in applications such as Graph Neural Networks (GNNs)~\cite{gespmm, lin2021accelerating}. We illustrate the SpMMul problem in Figure~\ref{fig:overall}(a), a typical dataflow of SpMMul is to calculate each element of the output matrix, $Y[m, n]$, by calculating the inner-product between the $m$-th row of $A$ and the $n$-th column of $X$. For each row of $A$, elements are sparsely distributed. Thus, corresponding elements in a column of $X$ are selected.

We summarize the dataflow with a sequential implementation for the SpMMul problem into three loops, as is shown in Figure~\ref{fig:overall}(b). The outermost loop is the $M$-Loop, which traverses rows of matrix $A$, specifying the row index $m$ of the output matrix $Y$, shown in Figure~\ref{fig:overall}(c). The next loop is the $N$-Loop, which traverses columns of $X$, specifying the column index $n$ of $Y$, shown in Figure~\ref{fig:overall}(d). Then, the innermost loop is the $K$-Loop, which traverses non-zero elements {$k_1^{(m)},k_2^{(m)},...,k_{K(m)}^{(m)}$} in $A$ and their corresponding elements in $X$, shown in Figure~\ref{fig:overall}(e). Parallelism exists in three loops. Optimizing SpMMul is then simplified into mapping these loops to parallel workers on GPUs (e.g., warps/threads) efficiently.

%Figure~\ref{fig:overall} illustrates the inner-product version of the dataflow of the SpMMul problem, and we will further use it to illustrate the design space throughout Section~\ref{sec:designspace}. This abstraction is generalized to outer-product dataflow in Section~\ref{sec-designspace-unify}, and we show that our statements of the design space remain valid.

%A naive parallel implementation of SpMMul based on GPUs can be described as followed: each thread computes one output in $Y$, which is the dot product of a sparse row vector of $A$ and a dense column vector of $X$. Threads within a warp are organized by unfolding M-Loop, which means threads in the same warp shares the same sparse row of $A$ and computes warpsize elements in the corresponding row of $Y$. $A$ and $X$ are stored in the global memory. Each non-zero element in $A$ is requested by N times, leadint to $nnz*N$ times of global requests. Each element in $X$ is requested by M times, leading to $M*N*K$ times of global requests, which adds up to a large number of global memroy access.

%\mentioned{Similar to a dataflow graph of a program, our graphic notation uses node to represent values and the operation which produces it, and edges to represent dataflow. Our notation however is distinctive from DFG because we use two types of dataflow, i.e., access indirection and computation. Access indirection, the dashed arrows in Fig.~\ref{fig:overall}, represents that loading the destination node value requires an address computed from the source node, i.e. an indirect load dependent on the source. Computation edges, the other arrows are the same as in the DFG, meaning the data dependency of arithmetic operations. As shown in the figure, SpMMul computation involves access indirection from the meta data of each non-zero element, to the corresponding value in the rhs matrix. The metadata itself can be indirectly accessed from the higher level of the data structure, e.g., pointers of the CSR format. The dataflow is the multiplication between non-zero and RHS values, and the sum reduction in the inner-product, which yields the final results.}


%\subsection{Related Works}\label{sec:baseline:relatedwork}






% \section{Optimization on SpMMul}\label{sec:baseline:opt}

% Previous works have proposed several optimization methods for SpMMul on GPUs, and we do a comprehensive survey on these methods in this section.

\subsection{SpMMul Optimizations}

\subsubsection{Shared Memory.}\label{sec:baseline:opt:sharedmemory}

%\textbf{Motivation:}
The shared memory is software-controlled scratchpad memory private to each thread block. Storing frequently-visited data into the shared memory for reuse can effectively reduce access latency and off-chip traffic.

\textbf{Approach:} In SpMMul, a sparse-matrix element $A[m,k]$ can be reused to multiply with different columns of the dense matrix, \textit{i.e.,} $X[k,n]$ for different $n$. To exploit this inter-thread reuse GE-SpMM~\cite{gespmm}, uses the following approach: First load sparse elements in the same row, $k_1^{(m)},...,k_{K(m)}^{(m)}$, altogether into the shared memory. Next, assign parallel threads to compute $Y[m, n]$ with different $n$ by iterating over the $k^{(m)}$'s in the shared memory, shown in Figure~\ref{fig:optimization}(a).

\textbf{Evaluation setup:} We evaluate this technique with a set of 27 sparse matrices, synthesized by R-MAT generator~\cite{chakrabarti2004r} with different matrix sizes, average row-length, and row-length variance. We use the open-source code of GE-SpMM~\cite{gespmm, codegespmm} and test on three GPUs described in Section~\ref{sec:exp:setup}.

\textbf{Results:} GE-SpMM's shared memory optimization improves performance on all 27 matrices and 3 GPUs, with average \textbf{1.20$\times$}, \textbf{1.32$\times$}, \textbf{1.13$\times$} on RTX 3090, RTX 2080, Tesla V100, respectively.

% In devices like Nvidia GPUs, the memory hierarchy can be simplified as followed: each thread has its private local memory, each thread block has shared memory which can be read and written by all the threads in the block, and all the threads on the device have access to the same global memory.

% Acting as a block-level cache for global memory, shared memory technique can be utilized to reduce the bandwidth consumption and improve the computational efficiency on such bandwidth-bounded scenarios. In SpMMul, each output in $Y$ is computed by the dot product of a sparse row vector of $A$ and a dense column vector of $X$, which is a large number of load requests. We can ensure regular access to the density matrix $X$, which is decided by the way we store the matrix(row-major or column-major), making it suitable for achieving high parallelism and bandwidth utilization. But the sparsity of matrix $A$ leads to irregular access patterns of global memory. By making threads within a warp loading the non-zero elements of $A$ into shared memory, we reduce the number of global memory loading requests by a factor of warp-size, which brings significant speedup on such bandwidth-limited scenario. The benefits of introducing shared memory is illustrated in figure \ref{fig:shm}. The average speedup by shared memory on ? graphs is 

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.48\textwidth]{figure/benefits_shared_memory.pdf}
%    \caption{speedup with shared memory technique on GTX 1080Ti and RTX 2080.}
%    \label{fig:shm}
%\end{figure}

\begin{figure*}[!tp]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/optimization.pdf}
    \vspace{-10pt}
    \caption{Previous SpMMul optimization on GPUs. (a) Shared Memory. (b) Thread Coarsening. (c) Vectorized Loading. (d) Tiling.}
    %\vspace{-10pt}
    \label{fig:optimization}
\end{figure*}


\subsubsection{Thread Coarsening.}\label{sec:baseline:opt:coarsening}

%\textbf{Motivation:}
By converting originally parallel workloads to a single sequential thread, one can re-use the loaded data as operands for more computation. This technique, named thread coarsening, reduces the amount of memory access. Prior work observes the memory bandwidth is saturated by excessive memory access when $N$ is large in SpMMul~\cite{gespmm}, which motivates the application of thread coarsening.

\textbf{Approach:} The thread coarsening optimization exploits the insight that sparse-matrix element $A[m,k]$ can be re-used for $Y[m,n]$ with different $n$, similar to the observation in the shared memory technique. Prior work~\cite{gespmm} makes each thread compute two output elements $Y[m,n]$ and $Y[m, n+D]$ where the stride $D$ is set, shown in Figure~\ref{fig:optimization}(b). 

\textbf{Evaluation setup:} We evaluate this technique with the same set of synthesized sparse matrices as in the previous subsection. We compare no-optimization (each thread computes one output element) with GE-SpMM's default implementation where each thread produces two output elements. 

\textbf{Results:} GE-SpMM's thread coarsening optimization brings speedup on 7, 25, and 10 matrices on three GPUs respectively, out of all 27 matrices. The technique causes \textbf{0.94$\times$, 0.98$\times$} degradation on Tesla V100 and RTX 3090, but gives average \textbf{1.20$\times$} speedup on RTX 2080 because RTX 2080 has relatively low memory bandwidth and is sensitive to traffic reduction optimizations. 
% Thread Coarsening is another technique commonly used on GPUs. Normally we want to exploit the highest parallelism when executing on GPUs, but it may lead to redundant memory access. Through thread coarsening, we can merge multiple threads into one, allowing re-use of data and reduce bandwidth consumption. If the task is bandwidth-bounded rather than computation-bounded, the increased memory efficiency may outweigh reduced parallelism and achieve better performance. 

\begin{table*}[!tp]
    \centering
    \vspace{-10pt}
    \caption{Review of optimizations for SpMMul on GPUs with controlled experiments (Min.-Avg.-Max.)}
    \vspace{-5pt}
      \begin{tabular}{c|c|c|c|c|c|c|c}
      \hline
      \multirow{2}[4]{*}{} & \multicolumn{4}{c|}{Reference}      & \multicolumn{3}{c}{Speedup w/ the optimization technique} \\
  \cline{2-8}          & \cite{hong2018efficient}   & \cite{aspt}, \cite{jiang2020novel}   & \cite{gespmm}   & \cite{sputnik}, \cite{wang2020sparsert}   & RTX 3090 & RTX 2080 & Tesla V100 \\
      \hline
      Shared memory & \checkmark   & \checkmark   & \checkmark   & \checkmark   & \underline{0.96}-1.20-1.68 & 1.09-1.32-2.02 & 1.03-1.13-1.36 \\
      Thread coarsening &       & \checkmark   & \checkmark   & \checkmark   & \underline{0.82}-\underline{0.98}-1.25 & \underline{0.61}-1.20-1.50 & \underline{0.75}-\underline{0.94}-1.20 \\
      Vertorized loading & \checkmark   &       &       & \checkmark   & 1.09-1.55-2.15 & 1.41-1.72-1.93 & \underline{0.92}-1.44-1.77 \\
      Tiling* & \checkmark   & \checkmark   &       &       & \underline{0.54}-\underline{0.86}-1.00 & \underline{0.63}-\underline{0.92}-1.06 & \underline{0.67}-\underline{0.91}-1.01 \\
      \hline
      \multicolumn{8}{l}{\small{*Use synthesized block-sparse matrices. Others use R-MAT matrices.}}\\
      \end{tabular}%
    \label{tab:opt}%
    \vspace{-5pt}
  \end{table*}%

\subsubsection{Vectorized Loading.}
%load连续的情况下，一个float2好于两个float

%\textbf{Motivation:}
Vectorized load instructions refer to loading 8 or 16 bytes per thread in one instruction, in form of \texttt{float2, float4}, etc. In applications with excessive random access, vector loading can increase the amount of effective data per request and improve bandwidth efficiency. 

\textbf{Approach:} Sputnik~\cite{sputnik,codesputnik} proposed careful designs to use vector loading for sparse and dense elements. Regarding sparse elements, if the sparse matrix rows are long enough to fill two \texttt{float}-load instructions, Sputnik uses \texttt{float2}-load combined with alignment techniques to load sparse rows efficiently. Regarding dense elements, vector loading can be applied to consecutive $X$ elements in a row.

\textbf{Evaluation setup:} Exploiting the aforementioned insight that each $A[m,k]$ can be used to multiply $X[k,n]$ for all $n$, we make a thread to loading $X[k,0],X[k,1]$ in form of \texttt{float2} if $X$ has a row-major layout, and compare it with the version using 2 \texttt{float} instructions. We implement this comparison on top of a classic SpMV implementation CSR-vector~\cite{bell2009implementing}, and test on the same matrix set as used in previous two subsections, shown in Figure~\ref{fig:optimization}(c).

\textbf{Results:} Vectorized loading brings \textbf{1.55$\times$}, \textbf{1.72$\times$}, \textbf{1.44$\times$} speedup on 3 GPUs respectively in the experiment described above. The vectorized loading benefits performance except for one case on Tesla V100 (0.92$\times$ degradation).

\subsubsection{Tiling.}
%\textbf{Motivation:}
Tiling can enhance the data re-use in matrix-multiplication and effectively reduce off-chip traffic. Coarse-grained tiling methods group sparse elements into 2-D grid to exploit the locality of the pointed dense tiles. Fine-grained sparse-matrix tiling is based on the insight that each dense element $X[k, n]$ can be re-used to multiply $A[m, k]$ with different $m$, and this re-use chance further reduces traffic for $X$.

\textbf{Approach:} Tiling the sparse matrix is challenging because retrieval of $A[m, k]$ with the same $k$ is difficult under row-wise compressed CSR format. ASpT~\cite{aspt} proposed to detect and mark the sparse-matrix elements belonging to the same column $k$. Through their special format, element $X[k, n]$ can be re-used for multiplying $A[m, k]$ with the same $k$ and different $m$, if the number of such $A[m, k]$ exceeds a threshold. The synchronization after collaboratively loading $X[k,:]$ into shared memory is the overhead of this optimization.

\textbf{Evaluation setup:} The sparse-matrix tiling proposed by ASpT~\cite{aspt} targets the sparsity pattern with vertical non-zero vectors, which rarely exists in random matrices generated by R-MAT. Thereby we evaluate this optimization on a set of 9 synthesized block-sparse matrices, with block size {8,16,32} and matrix size {1k, 4k, 20k}. We modify the source code~\cite{codeaspt} of ASpT to disable the preprocessing for comparison. 

\textbf{Results:} ASpT's approach brings speedup on 3, 5, 2 matrices on 3 GPUs, respectively, out of 9 matrices in the set. The average effect is \textbf{0.86$\times$}, \textbf{0.92$\times$}, \textbf{0.91$\times$} after applying the design, while in some cases the technique brings 1.06$\times$ speedup. %We confirm through this experiment that the sparse tiling technique needs to be applied selectively.
% Matrix tiling is a technique that is often utilized to reduce bandwidth and is of more efficiency when the data exhibit great spatial locality. The tiling technique loads the tiles from global memory into in-block shared memory and threads within a block will compute the tile in the same phase and then moves to the next phase to compute the next tile, as in the following matrix multiplication example.

% data reuse

\subsection{Motivation Summary}

Through reviewing previous work on SpMMul kernel design in Table~\ref{tab:opt}, we find that both improvement and degradation is observed from applying the same technique on different matrices or hardware. Thus, the static optimization cannot always lead to performance improvement, motivating our later designs in the following sections.

% Table generated by Excel2LaTeX from sheet 'Sheet1'

  

%\begin{table}[!h]
%    \caption{Review of Optimizations for SpMMul}
%    \centering
%    \small
%    \begin{tabular}{c|c|c|c|c}
%        \hline
%        Reference & shared memory & thread coarsening & vector loading & sparse matrix tiling \\
%        \hline 
%        \cite{hong2018efficient} & yes & & yes & yes \\
%        \cite{aspt}, \cite{jiang2020novel} & yes & yes & & yes \\
%        \cite{gespmm} & yes & yes & & \\
%        \cite{sputnik}, \cite{wang2020sparsert} & yes & yes & yes &  \\
%        \hline
%    \end{tabular}
%\end{table}

%\begin{table}[h]
%    \caption{Controlled Experiment on Effects of SpMMul Optimizations (Min.-Average-Max.)}
%    \centering 
%    \small 
%    \begin{tabular}{c|c|c|c}
%        \hline
%        Optimization & V100 & RTX2080 & RTX3090  \\ \hline
%        shared memory & 1.03-1.13-1.36 & 1.09-1.32-2.02 & 0.96-1.20-1.68 \\ \hline
%        thread coarsening & 0.75-0.94-1.20 & 0.61-1.20-1.50 & 0.82-0.98-1.25 \\ \hline
%        vector loading & 0.92-1.44-1.77 & 1.41-1.72-1.93 & 1.09-1.55-2.15 \\ \hline
%        sparse matrix tiling* & 0.67-0.91-1.01 & 0.63-0.92-1.06 & 0.54-0.86-1.00 \\ \hline
%        
%        \multicolumn{4}{l}{*Use synthesized block-sparse matrices. Others use R-MAT matrices.}\\
%        
%    \end{tabular}
%\end{table}

==> data/benchmark.tex <==


\section{Performance Analysis}\label{sec:benchmark}

In this section, we analyze how hardware parameters and data features affect the performance of different designs.


\begin{figure*}[!tp]
    \centering
    \includegraphics[width=\textwidth]{figure/classification.pdf}
    \vspace{-15pt}
    \caption{Importance of features (x-axis) to distinguish different designs. (a) RB and EB. (b) RM and CM. (c) SR and PR.}
    %\vspace{-15pt}
    \label{fig:classification}
\end{figure*}


\subsection{Visualization of Feature Importance}

To provide more insight on how input dynamics affect the performance, we train a variety of binary classification models using the same LightGBM method introduced in Section~\ref{sec:kernel}. Each binary classification problem is defined to classify two design choices in a dimension (\textit{i.e.,} RB/EB, RM/CM, SR/PR). The LightGBM model provides the importance metric to identify the importance of an input feature on the classification results. Thus, we train 4 binary classification models to select the better design for each dimension on one GPU ($3\times 4=12$ models for each dimension in total), with the importance of input features, shown in Figure~\ref{fig:classification}. 

\subsection{Analysis}

\subsubsection{RB and EB.} We can see in Figure~\ref{fig:classification}(a), \textit{std\_row} is the major factor to distinguish these two methods. We have analyzed in Section~\ref{sec:designspace:mloop} and Figure~\ref{fig:rb-eb}, a larger \textit{std\_row} leads to more imbalanced workloads among GPU workers. We show the relationship between \textit{std\_row} and performance ratio of EB/RB in Figure~\ref{fig:stdrow} for all matrices in the SuiteSparse dataset. We can observe a positive correlation in the figure, showing the same conclusion that a larger \textit{std\_row} leads to a higher performance ratio between EB and RB.

\begin{figure}[!tp]
    \centering
    \includegraphics[width=0.48\textwidth]{figure/stdrow-control.pdf}
    \vspace{-15pt}
    \caption{Relationship between \textit{std\_row} and performance ratio of EB/RB. We normalize \textit{std\_row} with average non-zeros in a row. X-axis: normalized \textit{std\_row}. Y-axis: EB/RB.}
    \vspace{-6pt}
    \label{fig:stdrow}
\end{figure}

\subsubsection{RM and CM.} We can see in Figure~\ref{fig:classification}(b) that these two methods cannot be easily distinguished by one certain feature. Features including \textit{std\_row}, \textit{nnz}, and \textit{mat\_size} share similar importance on the classification result. Although we have shown in Figure~\ref{fig:rm-cm}(c) that CM exceeds RM on synthesized matrices with controlled parameters, it hardly achieves better performance against RM on real-world matrices (less than 0.5\% in all scenarios in Figure~\ref{fig:ratio}). Thus, the importance of features in Figure~\ref{fig:classification}(b) is buried by the noise. RM and CM differ in the data access pattern to the dense matrix. Thus, we show the L2 cache hit ratio and the average number of sectors per request (a larger number of sectors means more data is accessed for one time) issues by L2 miss in Figure~\ref{fig:l2} ($N$=32). We show the difference between two groups of matrices (CM is faster than RM, and CM is slower). When CM is faster than RM, it achieves a higher L2 cache hit ratio. Moreover, due to coalesced loading, RM always has a larger number of sectors per request. However, when CM exceeds RM, the metric is improved by 11\% to 26\% for CM, while the difference between two RM groups is only 3\% to 5\%. Thus, CM achieves better performance when the memory access pattern is more coalesced.

\begin{figure}[!tp]
    \centering
    \includegraphics[width=0.45\textwidth]{figure/L2.pdf}
    \vspace{-5pt}
    \caption{Difference between two groups of matrices (CM faster than RM and CM slower than RM) on L2 cache metrics.}
    \vspace{-6pt}
    \label{fig:l2}
\end{figure}


\subsubsection{SR and PR.} We can see in Figure~\ref{fig:classification}(c), \textit{nnz} is the main factor to distinguish these two methods, which is also coordinated with our previous analysis in Section~\ref{sec:designspace:kloop} and Figure~\ref{fig:sr-pr}(c). When \textit{nnz} becomes larger, higher parallelism is required from the hardware perspective. To show how hardware parallelism affects the performance, we use NVIDIA CUDA MPS (Multi-Process Service)~\cite{nvidia2019mps} to set the percentage of CUDA cores when running an algorithm. The result is shown in Figure~\ref{fig:mps}, we run 4 algorithms and normalize the performance to using 10\% CUDA cores. Two RB algorithms achieve a higher performance improvement against two SR methods. The conclusion is aligned with our previous analysis, that PR benefits more from a higher GPU parallelism.
% A larger \textit{nnz} requires higher parallelism, and we further show the relationship between \textit{nnz} and the performance ratio of PR/SR in Figure~\ref{fig:stdrow} for all matrices in the SuiteSparse dataset. We can observe a negative correlation in the figure, showing the same conclusion that a larger \textit{nnz} leads to a better SR performance against PR.

% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figure/nnz-control.pdf}
%     \vspace{-15pt}
%     \caption{Relationship between \textit{nnz} and performance ratio of PR/SR. We normalize \textit{nnz} with the maximum non-zeros in a row. X-axis: normalized \textit{nnz}. Y-axis: PR/SR.}
%     \vspace{-5pt}
%     \label{fig:nnz}
% \end{figure}

%On the other hand, when \textit{nnz} becomes larger, the problem requires higher parallelism from the hardware perspective. To show how hardware parallelism affects the performance, we use NVIDIA CUDA MPS (Multi-Process Service)~\cite{nvidia2019mps} to set the percentage of CUDA cores when running a kernel. The result is shown in Figure~\ref{fig:mps}, we run 4 kernels and normalize the result to the performance of using 10\% CUDA cores. Two kernels based on RB achieve a higher performance improvement compared with two SR methods. The conclusion is aligned with our previous analysis, that PR benefits more from a higher GPU parallelism.




%\subsection{\todo{Benchmarks from hardware perspective}}






% In order to evaluate the performance of the SpMMul design, an unbiased and objective benchmark for the SpMMul problems is required. We present the methodology to design an unbiased and objective benchmark for SpMMul in both general-purpose and domain-specific scenarios.

% \subsection{General-Purpose Scenarios}\label{sec:benchmark:general}

% We implement SpMMul with different selects proposed in Section~\ref{sec:designspace}, and we get 8 static designs. According to the analysis in Section~\ref{sec:designspace:designspace}, one static design cannot always achieve the best performance for different input data. We show the performance of these 8 static designs in Figure~\ref{fig:order} (a)-(c), the detailed setup is in Section~\ref{sec:exp:setup}. The performance of each design is normalized to the best design and we sort the dataset for each design in Figure~\ref{fig:order}.

% Besides the conclusion that the performance is related to the input data characteristics, we can see a severe bias in the benchmark. As we can see in Figure~\ref{fig:order} (d)-(f), the RB+RM+SR design achieves the best performance in most cases, and four designs based on CM hardly win (according to our results, four CM-based designs only win on 0.23\% of all datasets.), this means that CM-based designs do not apply to natural sparse matrices (matrices in SuiteSparse~\cite{davis2011university} are from various domains) rather than synthesized matrices (e.g., matrices used in the controlled experiments in Section~\ref{sec:designspace:nloop}). However, for the other four designs based on RM, an unbiased benchmark for the general-purpose SpMMul should be balance for these designs. 

% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figure/order.pdf}
%     %\vspace{-20pt}
%     \caption{(a)-(c) Normalized performance to the best of 8 static designs proposed in Section~\ref{sec:designspace}. X-axis: different datasets after sorting for each implementation. Y-axis: normalized performance. (d)-(f) The percentage of datasets that one static design achieves the best performance.}
%     %\vspace{-10pt}
%     \label{fig:order}
%  \end{figure}

% Based on analysis above, we propose our benchmark, SpMBench, for SpMMul problems. SpMBench is consisted of 107 (matrix, $N$) pairs, where matrices are selected from SuiteSparse~\cite{davis2011university} and $N$ varies from 1 to 128. The list of SpMBench is anonymously listed online~\cite{spmbench}. Based on SpMBench, percentages of datasets that one static design achieves the best performance are balanced for the four RM-based designs, shown in Figure~\ref{fig:spmbench}. We also include (matrix, $N$) pairs that CM-based designs achieve the best performance to cover conner cases.

% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figure/spmbench.pdf}
%     %\vspace{-10pt}
%     \caption{The percentage of datasets that one static design achieves the best performance using our SpMBench. The legends are same with Figure~\ref{fig:order}.}
%     %\vspace{0pt}
%     \label{fig:spmbench}
%  \end{figure}



% \subsection{Domain-Specific Scenarios}\label{sec:benchmark:specific}

% The motivation of SpMBench is to cover different cases for SpMMul problems. We need to mention that the listed SpMMul is not the only benchmark for SpMMul problems, while it just targets at eliminating biases in previous datasets used for SpMMul designs. Besides, SpMMul kernels are widely used in many domain-specific scenarios, e.g., Graph Neural Networks (GNNs). In these scenarios, a benchmark for general-purpose SpMMul problems is not suitable. Previous works~\cite{gespmm} have mentioned that, GNNs usually use large $N$. GNNs can be used in various domains, e.g., citation networks~\cite{kipf2016semi} and traffic networks~\cite{yu2017spatio}. However, data in different domains show various characteristics which may lead to different performance on different designs. In order to test the performance of SpMMul design for a specific scenario, characteristics from a domain should be analyzed. We have shown in Figure~\ref{fig:order} that CM-based design cannot achieve better performance on natural graphs, thus we plot the performance comparison on other two dimensions in Figure~\ref{fig:gnnbenchmark}.

% We label matrices from three typical domains, including citation networks~\cite{SNAP}, traffic networks~\cite{SNAP}, and matrices in the control problems~\cite{VDOL}. As we can see, matrices from different domains lie in different area. Thus, we can use the coordinates to represent the performance characteristic of a matrix, and generate a performance benchmark for a specific domain by selecting neighbor matrices on the coordinate plain. For example, we only show 4 traffic network matrices, while we can get more matrices from other domains as the benchmark to test the performance of GNN systems on the traffic networks.

% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figure/gnnbenchmark.pdf}
%     %\vspace{-10pt}
%     \caption{Performance characteristics of matrices from different domains.}
%     %\vspace{-10pt}
%     \label{fig:gnnbenchmark}
%  \end{figure}


